Efficient size estimation and impossibility of termination in uniform dense population protocols

We study uniform population protocols: networks of anonymous agents whose pairwise interactions are chosen at random, where each agent uses an identical transition algorithm that does not depend on the population size $n$. Many existing polylog$(n)$ time protocols for leader election and majority computation are nonuniform: to operate correctly, they require all agents to be initialized with an approximate estimate of $n$ (specifically, the exact value $\lfloor \log n \rfloor$). Our first main result is a uniform protocol for calculating $\log(n) \pm O(1)$ with high probability in $O(\log^2 n)$ time and $O(\log^4 n)$ states ($O(\log \log n)$ bits of memory). The protocol is converging but not terminating: it does not signal when the estimate is close to the true value of $\log n$. If it could be made terminating, this would allow composition with protocols, such as those for leader election or majority, that require a size estimate initially, to make them uniform (though with a small probability of failure). We do show how our main protocol can be indirectly composed with others in a simple and elegant way, based on the leaderless phase clock, demonstrating that those protocols can in fact be made uniform. However, our second main result implies that the protocol cannot be made terminating, a consequence of a much stronger result: a uniform protocol for any task requiring more than constant time cannot be terminating even with probability bounded above 0, if infinitely many initial configurations are dense: any state present initially occupies $\Omega(n)$ agents. (In particular, no leader is allowed.) Crucially, the result holds no matter the memory or time permitted. Finally, we show that with an initial leader, our size-estimation protocol can be made terminating with high probability, with the same asymptotic time and space bounds.

==> proof-that-isolation-technique-does-not-work.tex <==
\begin{proof}
    Suppose for the sake of contradiction that $P$ is $\epsilon$-$\ninit$-$t$-terminating.
    Consider the initial configuration $\vi_{\ninit} \in I$ of size $\ninit$.
    The probability is $\epsilon$ that $P$ takes at least time $t(n)$ to reach from $\vi_{\ninit}$ to a terminated configuration $\vc$.
    Each execution $\xi$ resulting in a terminated configuration is finite,
    so there are a countable number of such executions $\xi_1,\xi_2,\ldots$,
    and $\sum_{i=1}^\infty \Pr[\xi_i] = \epsilon$.
    Order the executions by length.
    For some finite $m$,
    $\sum_{i=1}^m \Pr[\xi_i] \geq \epsilon / 2$.
    Let $\numinter = \max\limits_{1 \leq i \leq m} |\xi_i|$ be the length of the longest execution among these $m$.
    That is to say,
    with probability at least $\epsilon/2$,
    any execution of length $\numinter$ will result in a terminated configuration 
    (since it will have one of the $\xi_1\ldots,\xi_m$ as a prefix).
    
    Now consider a large initial configuration $\vi_n$ for $n > \ninit$.
    Consider the set of $u = \binom{n}{\ninit}$ subsets $S_1,\ldots,S_u$ of agents,
    each of size $\ninit$.
    Say that an interaction between two agents \emph{involves $S_i$} 
    if at least one agent is in $S_i$,
    and that the interaction is \emph{internal to $S_i$} if both agents are in $S_i$.
    For $i\in\{1,\ldots,u\}$,
    if the first $\numinter$ interactions involving $S_i$ are internal to $S_i$,
    we say that $S_i$ is \emph{isolated for $\numinter$ interactions}.
    Define the 0/1-indicator random variable $X_i$ for the event that $S_i$ is isolated for the first $\numinter$ interactions.    
    
    Let $Y_i$ be the 0/1-indicator random variable for the event 
    that the first $\numinter$ interactions %internal to 
    involving $S_i$ % have one of $\xi_1\ldots,\xi_m$ as a prefix 
    have a terminated agent.
    As indicated above,
    if $S_i$ is isolated for $\numinter$ interactions,
    then a terminated agent results with probability at least $\epsilon/2$,
    i.e., $\Pr[Y_i=1 | X_i=1] \geq \epsilon/2$.
    Therefore $\Pr[Y_i=1] \geq \Pr[Y_i=1 | X_i=1] \cdot \Pr[X_i=1] \geq \Pr[X_i=1] \cdot \epsilon/2$.
    
    To calculate $\Pr[X_i=1]$,
    we consider only interactions involving $S_i$.
    For each such interaction, 
    the probability that the other agent is in $S_i$ is $\frac{|S_i|-1}{n-1} = \frac{\ninit-1}{n-1}$.
    Since each interaction is independent,
    the probability that the first $\numinter$ such interactions are all internal is 
    $\Pr[X_i] = \left( \frac{\ninit-1}{n-1} \right)^\numinter$.
    So $\Pr[Y_i=1] \geq \left( \frac{\ninit-1}{n-1} \right)^\numinter \cdot \epsilon/2$.
    
    Define $X = \sum\limits_{i=1}^u X_i$,
    noting that $X > 0$ if and only if there exists a sub-population $S_i$ that is isolated for $\numinter$ interactions.
    By linearity of expectation,
    \begin{eqnarray*}
        \E[X] 
    &=& 
        \sum_{i=1}^u \E[X_i] 
    \\&=&
        u \cdot \left( \frac{\ninit-1}{n-1} \right)^\numinter
    \\&=&
        \binom{n}{\ninit} \cdot \frac{(\ninit-1)^\numinter}{(n-1)^\numinter}
    \\&<&
        e^\ninit \cdot \frac{n^{\ninit}}{\ninit^{\ninit}} \cdot \frac{(\ninit-1)^\numinter}{(n-1)^\numinter}
    \\&<&
        e^\ninit \cdot \frac{n^{\ninit}}{\ninit^{\ninit}} \cdot \frac{\ninit^{\numinter}}{n^{\numinter-1}}
    \\&=&
        e^\ninit \cdot n \cdot \left( \frac{\ninit}{n} \right)^{\numinter - \ninit}
    \end{eqnarray*}
    
    By Markov's inequality,
    $\Pr[X \geq 1] \leq \E[X] = e^\ninit \cdot n \cdot \left( \frac{\ninit}{n} \right)^{\numinter - \ninit}$.
    For example,
    for $\ninit=2$ and $\numinter = 4$,
    this is $e^2 \cdot n \cdot \left( \frac{2}{n} \right)^{4 - 2} = \frac{4 e^2}{n}.$
\end{proof}

==> sections/app-decay-sum-of-geometric.tex <==




==> sections/app-model.tex <==
\section{Model} \label{app:model}


\newcommand{\blank}{\llcorner\negthinspace\lrcorner}

\todoi{This whole section is a mess. Let's get something cleaner and less wordy.}

The system consists of a population of $n$ distributed and anonymous
(no unique IDs)
\emph{agents}, also called \emph{nodes} or \emph{processes}, that can perform local computations.
Each agent is a multitape ($r$-tape) Turing Machine which is defined by a $6$-tuple $M = \langle \Lambda, \Gamma, q_0, \epsilon, F, \delta \rangle$.
$\Lambda$ is a finite set of \emph{TM states},
%\todo{DD: I think we should allow blank in the tape alphabet. Or somehow indicate that the ability to tell where the end of the tape is has been ``built into the TM hardware''. Otherwise we have to talk about encodings of delimiters and it would get really ugly.}
$\Gamma$ is the binary \emph{tape alphabet} $\{0, 1\}$,
$q_0 \in \Lambda$ is the \emph{initial TM state},
% DD: elsewhere we use epsilon for empty string
% $\epsilon \in \Gamma$ is the blank symbol,
$F \subseteq \Lambda$  is the set of \emph{final TM states},
and $\delta: \Lambda \times \Gamma^r \rightarrow \Lambda \times (\Gamma \times \{L,R,S\})^r$ is the \emph{TM transition function}, where $L$ is left shift, $R$ is right shift and $S$ is no shift.
We assume that $r$ is a fixed constant, i.e. independent of the population size.

\todoi{There is no need for defining the work tape separately anymore. Since we changed the value of $\k$ to be a power of two, now we only require addition and shift for the computation.}
We define three types of tapes. \textit{Input}, \textit{Output} and \textit{Work} tapes. The Input and Output tapes provide information from and to the other agent during an interaction. The Work tapes are used for storing data and for internal operations, which can be assumed to be additions, subtractions and multiplications (divisions can be performed via the Euclidean Division Algorithm, which divides two integers using additions and subtractions).

\todo{$V$ is undefined here}
Let $r_i < r$ be the number of input tapes, $r_o < r$ the number of output tapes and $r_w < r$ the number of work tapes, where $r_i + r_o + r_w = r$.
For any $t \geq 0$ let $I(t), O(t)$ and $W(t)$ be $|V| \times r_i$, $|V| \times r_o$ and $|V| \times r_w$ matrices respectively, such that $I_{v,j}(t)$, $O_{v,j}(t)$ and $W_{v,j}(t)$ are the values of the $j$-th Input, Output and Work tapes respectively of the agent $v \in V$ at time $t$. Furthermore, for every $t \geq 0$, let $q(t)$ be a $|V|$-dimensional vector such that $q_{v}(t)$ is the \emph{state} (or \emph{agent-TM-configuration}) of $v \in V$ at time $t$.
We refer to $q(t)$ as the \emph{configuration} (or \emph{global-configuration}) at time $t$.
We say that a population protocol is \emph{leaderless} if $q_{v}(0) = q_0 \; \forall \; v \in V$, i.e.
all agents have the same state in the initial configuration.
We also say that $I(0)$ is the population input at time 0.

Let $S$ be the finite set of binary strings $\{0,1\}^*$.
This model is defined on a population $V$ of agents and consists of an
\emph{input initialization function}
$\iota : S \rightarrow S^r \times \Lambda$ and an
\emph{output function}
$\gamma : S^r \times \Lambda \rightarrow D$
($D$ is the set of output values).
Initially, the values of the tapes of each agent are determined by the input initialization function $\iota$, and in every step $t+1 \geq 1$, a pair of agents interacts.
During an interaction $(a, b)$ between two agents at time $t+1$, each agent updates its state and copies the contents of its Output tapes to the Input tapes of the other agent $(O_{a,:}(t) \rightarrow I_{b,:}(t+1)$ and $O_{b,:}(t) \rightarrow I_{a,:}(t+1))$.


==> sections/app-subexp.tex <==


\subsection{Subexponential random variables} \label{app:subexp}

The following lemma is well-known;
we prove it explicitly since the exact form is convenient for our purposes
but is more general than typically expressed.
It shows that exponential tail bounds for $\Pr{|X-\E{X}| > \lambda}$ 
give bounds on the moment-generating functions of the random variables $X-\E{X}$ and $\E{X}-X$.
The proof is modeled on Rigollet's proof of the analogous lemma for sub-gaussian random variables proven in~\cite{rigollet2015highdimensional}.

\todo{See if there's a way to avoid this ugliness with having two separate bounds. It's here because of the problem Eric pointed out, where $\E{X-\E{X}} = \E{\E{X}-X} = 0$, but $\E{|X-\E{X}|} \neq 0$.}

\begin{lemma}[\cite{rigollet2015highdimensional}] \label{lem:subexp-bound-mgf}
    Let $X$ be an $\alpha$-$\beta$-sub-exponential random variable.
    Then for all $s \in \left[ -\frac{1}{2\beta}, \frac{1}{2\beta} \right]$, 
    we have
    $\E{ e^{ s (X-\E{X}) } } , \E{ e^{ s (\E{X}-X) } } 
    \leq 1 + 2 \alpha \beta^2 s^2$.
\end{lemma}

\begin{proof}
    Let $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{|X - \E{X}|^k}
    &=&
        \int_0^\infty \Pr{|X - \E{X}|^k \geq \lambda} d\lambda
    =%\\&=&
        \int_0^\infty \Pr{|X - \E{X}| \geq \lambda^{1/k}} d\lambda
    \\&\leq&
        \int_0^\infty \alpha e^{- \lambda^{1/k} / \beta} d\lambda
    =%\\&=&
        \alpha \beta^k k \int_0^\infty e^{-u} u^{k-1} du  
        \ \ \ \ \ \ \text{substituting } u = \beta \lambda^{1/k}
    \\&=&
        \alpha \beta^k k \Gamma(k)
    =
        \alpha \beta^k k!,
    \end{eqnarray*}
    where $\Gamma(k)$ is the \emph{gamma function} 
    (defined by the given integral),
    known to equal $(k-1)!$ for $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{e^{s (X - \E{X}) }}
    &=&
        \E{ \sum_{k=0}^\infty 
        \frac{ ( s (X - \E{X}) )^k }{k!} } 
        \ \ \ \ \ \text{Taylor expansion of the exponential function}
    \\&=&
        \sum_{k=0}^\infty 
        \frac{ s^k \E{(X - \E{X})^k} }{k!} 
        \ \ \ \ \ \ \ \text{dominated convergence theorem}
    \\&=&
        1 + 
        s \underbrace{ \E{X - \E{X}} }_{= 0} + 
        \sum_{k=2}^\infty 
        \frac{ s^k \E{(X - \E{X})^k} }{k!}
    \\&\leq&
        1 + 
        \sum_{k=2}^\infty 
        \frac{ |s|^k \E{|X - \E{X}|^k} }{k!}
        \ \ \ \text{odd terms can only get larger}
    \\&\leq&
        1 + 
        \sum_{k=2}^\infty 
        \frac{ |s|^k \alpha \beta^k k! }{k!}
    =%\\&=&
        1 + 
        \alpha 
        \sum_{k=2}^\infty 
        \left( |s| \beta \right)^k
    =%\\&=&
        1 + 
        \alpha s^2 \beta^2
        \sum_{k=0}^\infty 
        \left( |s| \beta \right)^k
    \\&\leq&
        1 + \alpha \beta^2 s^2 \sum_{k=0}^\infty \frac{1}{2^k} 
        \ \ \ \ \ \ \ \ \ \ \ \text{since $|s| \leq \frac{1}{2 \beta}$}
    \\&=&
        1 + 2 \alpha \beta^2 s^2.
    \end{eqnarray*}
    The bound for $\E{ e^{ s (\E{X}-X) } }$
    is derived by a similar argument.
\end{proof}






The following Chernoff bound is similarly well-known,
but not stated in a convenient form in the existing literature,
so we prove a form that is convenient for our purposes.

\noindent
{\bf Lemma~\ref{lem:chernoff}}
\emph{\chernoffSubexpLemma}

% \begin{lemma}\label{lem:chernoff}
%     Let $\alpha,\beta > 0$ and $K \in \N^+$.
%     Let $X_1,\ldots,X_K$ be i.i.d. $\alpha$-$\beta$-sub-exponential random variables.
%     Define $X = \sum_{i=1}^K X_i$.
%     Then for all $\gamma \geq 0$,
%     $$
%         \Pr{|X - \E{X}| > \gamma \E{X} } 
%     \leq
%         2
%         \frac
%         { \left( 1 + \alpha / 2 \right)^K }
%         { e^{\gamma \E{X} / (2 \beta)} }.
%     $$
% \end{lemma}

\begin{proof}
    Then for all $t>0$,
    \begin{eqnarray*}
        \Pr{X - \E{X} > t}
    &=& 
        \Pr{e^{ s (X - \E{X}) } > e^{s t}} 
    \\&\leq& 
        \frac
        { \E{e^{s (X - \E{X}) } } } 
        { e^{s t} } 
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{Markov's inequality}
    \\&=&
        e^{- s t} 
        \E{ e^{ s \left( \left( \sum_{i=1}^K X_i \right) - \E{X} \right) } }
    \\&=&
        e^{- s t} 
        \E{ e^{ s \sum_{i=1}^K ( X_i  - \E{X_i} ) } }
        \ \ \ \ \text{linearity of expectation}
    \\&=& 
        e^{- s t} 
        \E{ \prod_{i=1}^K e^{s ( X_i - \E{X_i} ) } } 
    \\&=& 
        e^{- s t} 
        \prod_{i=1}^K 
        \E{ e^{s ( X_i - \E{X_i} ) } }. 
        \ \ \ \ \text{independence of the $X_i$'s}
    \end{eqnarray*}
    
    By Lemma~\ref{lem:subexp-bound-mgf},
    for all $|s| \leq \frac{1}{2\beta}$,
    $\E{ e^{s (X_i - \E{X_i}) } } \leq 1 + 2 \alpha \beta^2 s^2$.
    So
    $$
        \Pr{X - \E{X} > t} 
    \leq 
        e^{- s t }
        (1 + 2 \alpha \beta^2 s^2 )^K.
    $$
    
    Let $s = \frac{1}{2\beta}$. % and $t = \gamma \E{X}$.
    Then
    %\begin{eqnarray*}
    $$
        \Pr{ X - \E{X} > t }
    \leq %&\leq&
        e^{- s t}
        \left( 1 + 2 \alpha \beta^2 s^2 \right)^K
    = %\\&=&
        e^{- t / (2 \beta)}
        \left( 1 + \alpha / 2 \right)^K.
    % \\&=&
    %     e^{- \gamma \E{X} \beta / 2}
    %     \left( 1 + \frac{ K \alpha / 4} {K} \right)^K
    % \\&<&
    %     e^{- \gamma \E{X} \beta / 2}
    %     e^{- K \alpha / 4 }
    % \\&<&
    %     e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }
    %\end{eqnarray*}
    $$
    The proof that 
    $
        \Pr{ \E{X} - X \geq t } 
        % < e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }
        <
        e^{- t / (2 \beta)}
        \left( 1 + \alpha / 2 \right)^K
    $
    is symmetric.
    By the union bound,
    $
        \Pr{ |X-\E{X}| \geq t } 
    < 
        % 2 e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }.
        2 \cdot e^{- t / (2 \beta)}
        \left( 1 + \alpha / 2 \right)^K.
    $
\end{proof}







% \todoi{below here is not working}

% \todoi{We can (and should, for the sake of readers who would benefit from it) prove that the general case is sub-exponential for any $q$. We have to choose $\alpha$ large enough that $\alpha e^{-\lambda} > 1$ for $\lambda \leq 3$, to keep it above $\exp{-q^{3-\lambda}}$, which is close to 1 when $\lambda < 3$. But the following corollary is better than what we'd get for $q=\frac{1}{2}$ applied to that, so we should use the following. But it would help other people who stumble across this paper to see a sub-exponential tail bound for general maximum of geometric r.v.'s.

% Let's do this as a separate corollary to Lemma~\ref{lem:maxGeomTailBound}, and leave more Lemma~\ref{lem:maxGeomTailBound} and Corollary~\ref{cor:half-geom-is-sub-exp} as they are.

% The difficulty with showing $\exp{-q^{3-\lambda}} \leq \alpha e^{-\beta \lambda}$ for some $\alpha,\beta>0$ is the additive constant 3. We could say $\beta = q^3$, but this depends on $q$ and gets smaller as $q$ gets smaller. To get rid of the additive constant requires understanding the difference between $\E{X}$ and $\log_{1/q} n$ better, but it is complicated~\cite{eisenberg2008expectation}.}


% The following is a corollary of Lemma~\ref{lem:maxGeomTailBound},
% and it shows that the maximum of geometric random variables is sub-exponential. 
% %in the case $p \geq \frac{1}{e}$.
% It is weaker than Corollary~\ref{cor:half-geom-is-sub-exp} for the case of $p=q=\frac{1}{2}$,
% so we employ Corollary~\ref{cor:half-geom-is-sub-exp} for our main result.
% However, the analysis of the general case is a straightforward application of our existing techniques,
% so we include it in order to get a Chernoff bound for the sums of independent maxima of general geometric random variables,
% which may be useful in other contexts.

% \begin{corollary} \label{cor:max-geom-is-sub-exp}
%     Let $X_1,\ldots,X_n$ be i.i.d. $p$-geometric random variables,
%     $n \geq 2$,
%     let $q=1-p$,
%     and let $X = \max\limits_{1 \leq i \leq n} X_i$.
%     Then for all $\lambda > 0$,
%     $\Pr{ |X-\E{X}| \geq \lambda } \leq ?? e^{- \lambda \ln q}$,
%     i.e., $X$ is $\alpha$-$\beta$-sub-exponential for 
%     $\alpha = ??, \beta = \ln q$.
% \end{corollary}

% \begin{proof}
%     By Lemma~\ref{lem:maxGeomTailBound},
%     for all $\lambda > 0$,
%     $
%         \Pr{|X - \E{X}| < \lambda} 
%     < 
%         \exp{ - q^{3 - \lambda} }
%         + q^{\lambda}
%         + q^{2\lambda}
%     =
%         \exp{ - q^{3 - \lambda} }
%         + e^{\lambda \ln q}
%         + e^{2\lambda \ln q}
%     < 
%         \exp{ - q^{3 - \lambda} }
%         + 2 e^{\lambda \ln q}.
%     $
%     We complete the proof by bounding 
%     $\exp{ - q^{3 - \lambda} }$.
    
%     Write
%     $
%         \exp{ - q^{3 - \lambda} } = a \cdot \exp{- \frac{\lambda}{2} \ln q}.
%     $
%     Solving for $a$,
%     we get
%     $
%         a = \exp{q^{3-\lambda}} q^{\lambda / 2}
%     $
    
%     \begin{eqnarray*}
%         \exp{ - q^{3 - \lambda} }
%     &=&
%         \exp{ - q^{3} q^{-\lambda} }
%     \end{eqnarray*}
    
% \end{proof}

% \todoi{finish this}


==> sections/old-idea.tex <==
\section{Uniform protocols for size estimation and leader election}

A random variable $X$ is \emph{centered} if $\E{X}=0$.
For any random variable $X$ with finite expected value, 
define $c(X) = X - \E{X}$ to be the \emph{centering} of $X$.

% \begin{definition}[\cite{rigollet2015highdimensional}]
%     Let $\lambda>0$.
%     A centered random variable $X$ is \emph{$\lambda$-sub-exponential}
%     if for all $t \in \R$,
%     $\Pr{X > \E{X} + t} \leq 2 e^{-2t/\lambda}$.
% \end{definition}

\begin{definition}
    Let $\alpha,\beta>0$.
    A random variable $X$ is \emph{$\alpha$-$\beta$-sub-exponential}
    if for all $t \geq 0$,
    $\Pr{|X - \E{X}| \geq t} \leq \alpha e^{-\beta t}$.
\end{definition}

% The following consequence for the moment-generating function of a sub-exponential variable is useful.
% Sometimes the conclusion is taken as the definition of sub-exponential.

% \begin{lemma}[\cite{rigollet2015highdimensional}]
%     If $X$ is $\lambda$-sub-exponential,
%     then for all $s \leq \frac{1}{2\lambda}$, 
%     $\E{e^{sX}} \leq e^{2 s^2 \lambda^2}$.
% \end{lemma}

The following is restated in a way more conducive to our usage.
The proof is modeled on Rigollet's proof of the analogous lemma for sub-gaussian random variables proven in~\cite{rigollet2015highdimensional}.

\begin{lemma}[\cite{rigollet2015highdimensional}] \label{lem:subexp-bound-mgf}
    If $X$ is a $\alpha$-$\beta$-sub-exponential random variable,
    %with mean $\mu = \E{X}$,
    if $0 < s \leq \beta/2$, 
    then
    % $\E{e^{sX}} \leq e^{2 \alpha s^2 / \beta^2}$.
    $\E{ e^{ s (X-\E{X}) } } \leq 1 + 2 \alpha s / \beta$.
    and
    $\E{e^{s X}} \leq ???$.
\end{lemma}

\begin{proof}
    First we show the bound on $\E{ e^{ s (X-\E{X}) } }$.
    Let $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{|X - \E{X}|^k}
    &=&
        \int_0^\infty \Pr{|X - \E{X}|^k \geq t} dt
    =%\\&=&
        \int_0^\infty \Pr{|X - \E{X}| \geq t^{1/k}} dt
    \\&\leq&
        \int_0^\infty \alpha e^{-\beta t^{1/k}} dt
    =%\\&=&
        \alpha \frac{1}{\beta^k} k \int_0^\infty e^{-u} u^{k-1} du  \ \ \ \ \ \ \text{substituting } u = \beta t^{1/k}
    \\&=&
        \frac{\alpha}{\beta^k} k \Gamma(k)
    =
        \frac{\alpha}{\beta^k} k!
    \end{eqnarray*}
    
    \noindent
    Then
    \begin{eqnarray*}
        \E{e^{s(X - \E{X})}}
    &=&
        \E{ 1 + \sum_{k=1}^\infty \frac{ s^k (X - \E{X})^k }{k!} } \ \ \ \ \ \text{Taylor expansion of the exponential function}
    \\&=&
        1 + \sum_{k=1}^\infty \frac{ s^k \E{(X - \E{X})^k} }{k!} \ \ \ \ \ \ \ \text{dominated convergence theorem}
    \\&\leq&
        1 + \sum_{k=1}^\infty \frac{ s^k \E{|X - \E{X}|^k} }{k!} \ \ \ \ \ \ \ \text{negative terms become positive}
    \\&\leq&
        1 + \sum_{k=1}^\infty \frac{ s^k \frac{\alpha}{\beta^k} k! }{k!}
    =%\\&=&
        1 + \alpha \sum_{k=1}^\infty \left( \frac{s}{\beta} \right)^k
    =%\\&=&
        1 + \alpha \frac{s}{\beta} \sum_{k=0}^\infty \left( \frac{s}{\beta} \right)^k
    \\&\leq&
        1 + \alpha \frac{s}{\beta} \sum_{k=0}^\infty \frac{1}{2^k} \ \ \ \ \ \ \ \ \ \ \ \text{since $s \leq \frac{\beta}{2}$}
    \\&=&
        1 + 2 \alpha s / \beta. %\qedhere
    % \leq%\\&\leq&
    %     e^{2 \alpha s^2 / \beta^2}. \qedhere
    \end{eqnarray*}
    
    Now we show the bound on $\E{e^{s X}}$.
    TODO nonsense below here
    
    Let $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{|X - \E{X}|^k}
    &=&
        \int_0^\infty \Pr{|X - \E{X}|^k \geq t} dt
    =%\\&=&
        \int_0^\infty \Pr{|X - \E{X}| \geq t^{1/k}} dt
    \\&\leq&
        \int_0^\infty \alpha e^{-\beta t^{1/k}} dt
    =%\\&=&
        \alpha \frac{1}{\beta^k} k \int_0^\infty e^{-u} u^{k-1} du  \ \ \ \ \ \ \text{substituting } u = \beta t^{1/k}
    \\&=&
        \frac{\alpha}{\beta^k} k \Gamma(k)
    =
        \frac{\alpha}{\beta^k} k!
    \end{eqnarray*}
\end{proof}

%The next lemma's proof is modeled on Rigollet's proof of the analogous lemma for sub-gaussian random variables proven in~\cite{rigollet2015highdimensional}.

\todoi{The following lemma is where everything breaks with the ``centered'' r.v.'s. The idea of measuring $\Pr{|X-\E{X}| \geq t}$ is that this is an upper tail bound and a lower tail bound at the same time. However, the following argument is one-sided: the maximum over all $X_i$ exceeds $t$ if and only if there exists $i$ such that $X_i$ exceeds $t$ but there's no similar characterization for being less.

Also, even the other bound seems to break when I write it out as $X - \E{X} \geq t$... I'm so confused.}

\begin{lemma}\label{lem:max}
    Let $X_1,\ldots,X_n$ be independent $\alpha$-$\beta$-sub-exponential random variables,
    and let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then
    for all $t > 0$,
    $\Pr{|X-\E{X}| \geq t} \leq \alpha n e^{-\beta t}$.
\end{lemma}

\begin{proof}
    We consider the two cases: 
    \begin{description}
    \item[$X-\E{X} \geq t$:]
        By the union bound,
        $\Pr{X - \E{X} \geq t} 
        = \Pr{ (\exists i) X_i - \E{X} \geq t }
        \leq
        \sum\limits_{i=1}^n \Pr{X_i - \E{X} \geq t} %\ \ \ \ \text{union bound}
        \leq
        \alpha n e^{-\beta t}.$    
        
    \item[$X-\E{X} \leq -t$:]
        TODO
    \end{description} 
\end{proof}

We take the convention that $G_p$ is a \emph{$p$-geometric random variable}
if it is the number of consecutive $T$'s before the first $H$,
when flipping a coin with $\Pr{H}=p$
(not counting the flip that results in the first $H$).
Thus $\E{G_p} = \frac{1}{p} - 1$,
and for all $t \in \N$, 
$\Pr{G_p \geq t} = (1-p)^{t+1}$.
In particular $\E{G_{1/2}} = 1$.

\begin{corollary} \label{cor:maxGeomTailBound}
    Let $X_1,\ldots,X_n$ be i.i.d. $\frac{1}{2}$-geometric random variables,
    and let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then for all $t \in \N$,
    $\Pr{ |X-\E{X}| \geq t } \leq \frac{n}{2} e^{-t \ln 2}$.
\end{corollary}

\begin{proof}
    % Recall $c(X_i) = X_i - \E{X_i} = X_i - 1$ is the centering of $X_i$.
    % For each $t \in \N$, we have 
    % $
    % \Pr{c(X_i) \geq t}
    % = \Pr{X_i \geq t+1} 
    % = 2^{-(t+1)} 
    % = e^{-(t+1) \ln 2}
    % = e^{- \ln 2} e^{-t \ln 2}
    % = \frac{1}{2} e^{-t \ln 2}$.
    
    % Thus $c(X_i)$ is $\alpha$-$\beta$-sub-exponential for 
    % $\alpha = 1/2$ and $\beta=\ln 2$.
    % Applying Lemma~\ref{lem:max} to $c(X)$,
    % we have that for all $t > 0$,
    % $\Pr{X \geq \E{X} + t} 
    % = \Pr{c(X) \geq t} 
    % \leq \alpha n e^{-\beta t}
    % = \frac{n}{2} e^{-t \ln 2}$.
    
    For each $t \in \N$, 
    since $c(X_i)$ takes values in $-1,0,1,2,\ldots$,
    we have 
    $
    \Pr{|c(X_i)| \geq t}
    = \Pr{X_i \geq t+1}
    = 2^{-(t+1)} 
    = e^{-(t+1) \ln 2}
    = e^{- \ln 2} e^{-t \ln 2}
    = \frac{1}{2} e^{-t \ln 2}$.
    Thus $c(X_i)$ is $\alpha$-$\beta$-sub-exponential for 
    $\alpha = \frac{1}{2}$ and $\beta=\ln 2$.
    
    Note that 
    $c(X) 
    = \max\limits_{1 \leq i \leq n} c(X_i)$.
    Applying Lemma~\ref{lem:max} to $c(X_1),\ldots,c(X_n)$,
    we have that for all $t > 0$,
    $\Pr{|c(X)| \geq t} 
    \leq \alpha n e^{-\beta t}
    = \frac{n}{2} e^{-t \ln 2}$.
\end{proof}

Applying Lemma~\ref{lem:subexp-bound-mgf} 
with $\alpha = \frac{n}{2}$ and $\beta = \ln 2$ 
gives the following corollary.

\begin{corollary} \label{cor:maxGeomSubExp}
    Let $X_1,\ldots,X_n$ be i.i.d. $\frac{1}{2}$-geometric random variables,
    let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then 
    for all $|s| \leq \ln(2)/2$, 
    % $\E{e^{s c(X)}} \leq e^{n s^2 / \ln^2 2}$.
    $\E{ e^{ s |c(X)| } } \leq 1 + n \frac{s^2}{\ln^2 2}$.
    
\end{corollary}

\begin{lemma}\label{lem:bernstein}
    Let  $n,K \in \N^+$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then for all $\gamma \geq 0$,
    $\Pr{|X - \E{X}| > \gamma \E{X} } \leq ??$
\end{lemma}

\todoi{I really screwed up the reasoning about centered r.v.'s here. Not sure how to fix it.}

\begin{proof}
    By Markov's inequality and independence and the fact that $c(X_i) \geq -1$, % of the $X_i$'s,
    for all $s>0$ and $t \geq 1$,
    \begin{eqnarray*}
        \Pr{|X - \E{X}| > t}
    &=& 
        \Pr{e^{ s |X - \E{X}| } > e^{s t}} 
    \\&\leq& 
        \frac{ \E{e^{s |X - \E{X}|}} } { e^{s t} } 
    \\&=& 
        e^{- s t} \E{ e^{ \left| \left( \sum_{i=1}^K s X_i \right) - \E{X} \right| } }
    \\&=& 
        e^{- s t} \E{ e^{ \left| \left( \sum_{i=1}^K s X_i \right) - \sum_{i=1}^K \E{X_i} \right| } }
    \\&=& 
        e^{- s t} \prod_{i=1}^K \frac{ \E{ e^{s |X_i| } } } { \E{X_i} }.
    \end{eqnarray*}
    %
    % For each $1 \leq i \leq K$,
    % define $X_i' = X_i - \E{X_i}$ to be the centered version of $X_i$.
    By Corollary~\ref{cor:maxGeomSubExp},
    for all $|s| \leq \ln(2)/2$,
    $\E{ e^{ s |c(X_i)| } } \leq 1 + n \frac{s^2}{\ln^2 2}$.
    So
    $$
        \Pr{|c(X)| > t} 
        \leq e^{- s t} \prod_{i=1}^K \left( 1 + n \frac{s^2}{\ln^2 2} \right)
        = e^{- s t} \left( 1 + n \frac{s^2}{\ln^2 2} \right)^K
        %= e^{-st + K n s^2 / \ln^2 2}.
    $$
    %
    
    Let $H_n = \sum_{i=1}^n \frac{1}{n}$ be the $n$'th harmonic number,
    recalling that $\ln n < H_n < \ln n + 1$.
    It is known~\cite{eisenberg2008expectation} that 
    $H_n < \E{X_i} < H_n + 1$,
    so $H_n - 1 < \E{c(X_i)} < H_n$.
    By linearity of expectation,
    $\E{c(X)} > K (H_n - 1) > K (\ln n - 1)$.
    
    Let $s = \frac{\ln(2)}{2} > 1/3$ and $t = (1 + \gamma) \E{c(X)}$.
    Then
    \begin{eqnarray*}
        \Pr{|c(X)| > (1 + \gamma) \E{X}} 
    &\leq&
        e^{- s t} 
        \left( 1 + n \frac{s^2}{\ln^2 2} \right)^K
    \\&=&
        e^{- (1 + \gamma) \E{X} \frac{\ln(2)}{2}}  
        \left( 1 + n \frac{(\frac{\ln 2}{2})^2}{\ln^2 2} \right)^K
    \\&=&
        e^{- (1 + \gamma) \E{X} \frac{\ln(2)}{2}}  
        \left( 1 + \frac{n}{4} \right)^K
    \\&<& 
        e^{- (1 + \gamma) K \ln(n) / 3}
        \left( 1 + \frac{n}{4} \right)^K
    \\&=& 
        \left( e^{- (1 + \gamma) \ln(n) / 3} \left( 1 + \frac{n}{4}\right) \right)^K
    \\&=& 
        \left( n^{- (1 + \gamma) / 3} \left( 1 + \frac{n}{4}\right) \right)^K
    \\&<& 
        \left( n^{- (1 + \gamma) / 3} \left( \frac{n}{3} \right) \right)^K
    \\&=& 
        \left( \frac{1}{3 n^{(1 + \gamma) / 3 - 1}} \right)^K
    \end{eqnarray*}
\end{proof}


\begin{lemma} \label{lem:ave-geom-max}
    Let  $n,K \in \N^+$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then for all $\gamma \geq 0$,
    $\Pr{|X-\E{X}| > \gamma \E{X}} \leq ??$
\end{lemma}

\begin{proof}
    For each $X_i$, define $X_i' = X_i - \E{X_i}$ to be its centered version.
    Similarly define $X' = X - \E{X}$.
    By Corollary~\ref{cor:maxGeomSubExp},
    each $X_i'$ is $\alpha'$-$\beta$-sub-exponential for 
    $\alpha' = n / 4$
    and
    $\beta = \ln 2$.
    Applying Lemma~\ref{lem:bernstein} gives
    $\Pr{X - \E{X} > t} = \Pr{X' > t} \leq e^{K n / 16 - t \ln(2) / 2}$
    \todo{need some calculation of $\E{X}$}
    
    From here: \url{https://www.sciencedirect.com/science/article/pii/S0167715207002040}
    we have that $H_K < \E{X} < 1 + H_K$,
    where $H_n = \sum_{i=1}^K \frac{1}{K}$ is the $K$'th harmonic number.
\end{proof}

==> sections/old/geometric.tex <==
\subsection{Chernoff bound on sums of maxima of geometric random variables}
\label{subsec:geom}

% \todoi{
%     Looking into ``subexponential'' random variables for possibly proving tail inequalities on maximums of geometric random variables: 
    
%     \url{https://www.stat.berkeley.edu/~mjwain/stat210b/Chap2_TailBounds_Jan22_2015.pdf}
    
%     \url{http://tinyurl.com/y8r772hv}
    
%     This paper shows that geometric r.v.'s are sub-exponential: 
%     \url{https://arxiv.org/pdf/1301.3321.pdf}
    
%     This shows how to bound the maximum of sub-gaussian; perhaps we can imitate the proof for sub-exponential: 
%     \url{https://ocw.mit.edu/courses/mathematics/18-s997-high-dimensional-statistics-spring-2015/lecture-notes/MIT18_S997S15_Chapter1.pdf}
% }

\subsubsection{Sub-exponential random variables}

\begin{definition}
    Let $\alpha,\beta > 0$ and let $X$ be a random variable.
    We say $X$ is \emph{$\alpha$-$\beta$-sub-exponential} if,
    for all $\lambda>0$,
    $\Pr{X \geq \lambda} \leq \alpha e^{-\beta \lambda}$.
\end{definition}

The following lemma is well-known;
we prove it explicitly since the exact form is convenient for our purposes
but is more general than typically expressed.
It shows that exponential tail bounds $\Pr{|X-\E{X}| > \lambda}$ on a random variable $X$ give bounds on the moment-generating functions of the random variables $X-\E{X}$ and $\E{X}-X$.
The proof is modeled on Rigollet's proof of the analogous lemma for sub-gaussian random variables proven in~\cite{rigollet2015highdimensional}.

\todo{See if there's a way to avoid this ugliness with having two separate bounds. It's here because of the problem Eric pointed out, where $\E{X-\E{X}} = \E{\E{X}-X} = 0$, but $\E{|X-\E{X}|} \neq 0$.}

\begin{lemma}[\cite{rigollet2015highdimensional}] \label{lem:subexp-bound-mgf}
    Let $X$ be an $\alpha$-$\beta$-sub-exponential random variable.
    Then for all $s \in [-\beta/2, \beta/2]$, 
    we have
    $\E{ e^{ s (X-\E{X}) } } , \E{ e^{ s (\E{X}-X) } } 
    \leq 1 + 2 \alpha s^2 / \beta^2$.
\end{lemma}

\begin{proof}
    Let $k \in \N^+$.
    Then
    \todoi{MHS: either change $\lambda$ to $t$ or $t$ to $\lambda$}
    \begin{eqnarray*}
        \E{|X - \E{X}|^k}
    &=&
        \int_0^\infty \Pr{|X - \E{X}|^k \geq \lambda} dt
    =%\\&=&
        \int_0^\infty \Pr{|X - \E{X}| \geq \lambda^{1/k}} dt
    \\&\leq&
        \int_0^\infty \alpha e^{-\beta \lambda^{1/k}} dt
    =%\\&=&
        \alpha \frac{1}{\beta^k} k \int_0^\infty e^{-u} u^{k-1} du  
        \ \ \ \ \ \ \text{substituting } u = \beta \lambda^{1/k}
    \\&=&
        \frac{\alpha}{\beta^k} k \Gamma(k)
    =
        \frac{\alpha}{\beta^k} k!,
    \end{eqnarray*}
    where $\Gamma(k)$ is the \emph{gamma function} 
    (defined by the given integral),
    known to equal $(k-1)!$ for $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{e^{s (X - \E{X}) }}
    &=&
        \E{ \sum_{k=0}^\infty 
        \frac{ ( s (X - \E{X}) )^k }{k!} } 
        \ \ \ \ \ \text{Taylor expansion of the exponential function}
    \\&=&
        \sum_{k=0}^\infty 
        \frac{ s^k \E{(X - \E{X})^k} }{k!} 
        \ \ \ \ \ \ \ \text{dominated convergence theorem}
    \\&=&
        1 + 
        s \underbrace{ \E{X - \E{X}} }_{= 0} + 
        \sum_{k=2}^\infty 
        \frac{ s^k \E{(X - \E{X})^k} }{k!}
    \\&\leq&
        1 + 
        \sum_{k=2}^\infty 
        \frac{ |s|^k \E{|X - \E{X}|^k} }{k!}
        \ \ \ \text{odd terms can only get larger}
    \\&\leq&
        1 + 
        \sum_{k=2}^\infty 
        \frac{ |s|^k \frac{\alpha}{\beta^k} k! }{k!}
    =%\\&=&
        1 + 
        \alpha 
        \sum_{k=2}^\infty 
        \left( \frac{|s|}{\beta} \right)^k
    =%\\&=&
        1 + 
        \alpha \frac{s^2}{\beta^2} 
        \sum_{k=0}^\infty 
        \left( \frac{|s|}{\beta} \right)^k
    % \\&=&
    %     1 + 
    %     \alpha \frac{s^2}{\beta^2} 
    %     \frac{1}{1 - |s|/\beta}
    \\&\leq&
        1 + \alpha \frac{s^2}{\beta^2} \sum_{k=0}^\infty \frac{1}{2^k} 
        \ \ \ \ \ \ \ \ \ \ \ \text{since $|s| \leq \frac{\beta}{2}$}
    \\&=&
        1 + 2 \alpha s^2 / \beta^2.
    \end{eqnarray*}
    The bound for $\E{ e^{ s (\E{X}-X) } }$
    is derived by a similar argument.
\end{proof}






The following Chernoff bound is similarly well-known,
but not stated in a convenient form in the existing literature,
so we prove a form that is convenient for our purposes.

\begin{lemma}\label{lem:chernoff}
    Let $\alpha,\beta > 0$ and $K \in \N^+$.
    Let $X_1,\ldots,X_K$ be i.i.d. $\alpha$-$\beta$-sub-exponential random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then for all $\gamma \geq 0$,
    $$
        \Pr{|X - \E{X}| > \gamma \E{X} } 
    \leq
        2
        \frac
        { \left( 1 + \alpha / 2 \right)^K }
        { e^{\gamma \E{X} \beta / 2} }.
    $$
\end{lemma}

\begin{proof}
    Then for all $t>0$,
    \begin{eqnarray*}
        \Pr{X - \E{X} > t}
    &=& 
        \Pr{e^{ s (X - \E{X}) } > e^{s t}} 
    \\&\leq& 
        \frac
        { \E{e^{s (X - \E{X}) } } } 
        { e^{s t} } 
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{Markov's inequality}
    \\&=&
        e^{- s t} 
        \E{ e^{ s \left( \left( \sum_{i=1}^K X_i \right) - \E{X} \right) } }
    \\&=&
        e^{- s t} 
        \E{ e^{ s \sum_{i=1}^K ( X_i  - \E{X_i} ) } }
        \ \ \ \ \text{linearity of expectation}
    \\&=& 
        e^{- s t} 
        \E{ \prod_{i=1}^K e^{s ( X_i - \E{X_i} ) } } 
    \\&=& 
        e^{- s t} 
        \prod_{i=1}^K 
        \E{ e^{s ( X_i - \E{X_i} ) } }. 
        \ \ \ \ \text{independence of the $X_i$'s}
    \end{eqnarray*}
    
    By Lemma~\ref{lem:subexp-bound-mgf},
    for all $|s| \leq \frac{\beta}{2}$,
    $\E{ e^{s (X_i - \E{X_i}) } } \leq 1 + 2 \alpha s^2 / \beta^2$.
    So
    $$
        \Pr{X - \E{X} > t} 
    \leq 
        e^{- s t }
        (1 + 2 \alpha s^2 / \beta^2)^K.
    $$
    
    Let $s = \frac{\beta}{2}$ and $t = \gamma \E{X}$.
    Then
    \begin{eqnarray*}
        \Pr{ X - \E{X} > \gamma \E{X} }
    &\leq&
        e^{- s t}
        \left( 1 + 2 \alpha s^2 / \beta^2 \right)^K
    \\&=&
        e^{- \gamma \E{X} \beta / 2}
        \left( 1 + \alpha / 2 \right)^K.
    % \\&=&
    %     e^{- \gamma \E{X} \beta / 2}
    %     \left( 1 + \frac{ K \alpha / 4} {K} \right)^K
    % \\&<&
    %     e^{- \gamma \E{X} \beta / 2}
    %     e^{- K \alpha / 4 }
    % \\&<&
    %     e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }
    \end{eqnarray*}
    The proof that 
    $
        \Pr{\E{X} - X \geq \gamma \E{X}} 
        % < e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }
        e^{- \gamma \E{X} \beta / 2}
        \left( 1 + \alpha / 2 \right)^K
    $
    is symmetric.
    By the union bound,
    $
        \Pr{|X-\E{X}| \geq \gamma \E{X}} 
    < 
        % 2 e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }.
        2 e^{- \gamma \E{X} \beta / 2}
        \left( 1 + \alpha / 2 \right)^K.
    $
\end{proof}
























\subsubsection{Geometric random variables and their maximum}

We say $X$ is a \emph{$p$-geometric random variable}
if it is the number of consecutive $T$'s before the first $H$,
when flipping a coin with $\Pr{H}=p$
(\emph{not} counting the flip that results in the first $H$).
Thus $\E{X} = \frac{1}{p} - 1$;
in particular $\E{X} = 1$ if $p = \frac{1}{2}$.

The next lemma shows a tail bound on a maximum of geometric random variables.

\todoi{DD: see if we can change $q^{3 - \lambda}$ to $q^{2 - \lambda}$ by substituting $\Pr{|X-\E{X}| > \lambda}$ for $\Pr{|X-\E{X}| \geq \lambda}$. It seems okay to do as long as we track it through the proof of the sub-exponential lemma, but it seems strange to do since these are integer-valued random variables and it seems cleanest to use $\geq$}

\begin{lemma} \label{lem:maxGeomTailBound}
    Let $X_1,\ldots,X_n$ be i.i.d. $p$-geometric random variables,
    $n \geq 2$,
    let $q=1-p$,
    and let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then for all $\lambda > 0$,
    $
        \Pr{ \E{X}-X \geq \lambda } 
    \leq 
        \exp{ - q^{3 - \lambda} }
    $
    and
    $
        \Pr{ X-\E{X} \geq \lambda } 
    \leq 
        q^{\lambda} + q^{2\lambda}.
    $
\end{lemma}

\begin{proof}
    For each $t \in \N$, 
    $
        \Pr{X_i \geq t}
        = q^{t}
    $,
    so
    $
        \Pr{X_i \leq t}
        = 1 - \Pr{X_i \geq t+1}
        = 1 - q^{t+1}.
    $
    
    Since the $X_i$'s are independent,
    $
        \Pr{X \leq t} 
        = \prod_{i=1}^n \left( 1 - q^{t+1} \right)
        = \left( 1 - q^{t+1} \right)^n.
    $
    
    Let $H_n = \sum_{i=1}^n \frac{1}{n}$ be the $n$'th harmonic number,
    recalling that $\ln n < H_n < \ln n + 1$.
    It is known~\cite{eisenberg2008expectation} that 
    $\frac{1}{\lambda} H_n \leq \E{X} < \frac{1}{\lambda} H_n + 1$,
    where $q = e^{-\lambda}$.
    So $\lambda = - \ln q$,
    implying
    \todo{The second inequality here is not correct. It is more like $\E{X} < \log_{1/q} n + 1 + \ln \frac{1}{q}$, which can get large for $q$ close to 0. It is correct for $q=2$, since $\ln \frac{1}{q} \approx 0.693$}
    $\log_{1/q} n < \E{X} < \log_{1/q} n + 2$.
    \todoi{MHS: The todo on the right side seems wrong, because the second inequality would be like $\E{X} < \log_{1/q} n + 1 + \frac{1}{\ln \frac{1}{q}}$. So, even for $q=1/2$ it is more than $2$.}
% Got the next lemma from here:
% \url{https://math.stackexchange.com/questions/259543/rate-of-convergence-of-left1-fracax-rightx-to-operatornameexpa}
% I was really guessing at a lot of this; it will need to be fixed.

% Or we could just use this: \url{http://www.lkozma.net/inequalities_cheat_sheet/ineq.pdf}
% which states $(1+\frac{x}{n})^n \geq e^x (1 - \frac{x^2}{n})$.

    Below we use the inequalities
    $e^x \left( 1 - \frac{x^2}{n} \right) 
    \leq \left( 1+\frac{x}{n} \right)^n 
    \leq e^x$
    for $n > 1, |x| < n$.

    Setting $t = \E{X} - \lambda$, we have
    \begin{eqnarray*}
        \Pr{X \leq \E{X} - \lambda}
    &=&
        \left( 1 - q^{t + 1} \right)^n
    \\&=&
        \left( 1 - q^{(\E{X} - \lambda) + 1} \right)^n
    \\&<&
        \left( 1 - q^{\log_{1/q} n + 2 - \lambda + 1} \right)^n
    \\&=&
        \left( 1 - q^{\log_{1/q} n} q^{3 - \lambda} \right)^n
    \\&=&
        \left( 1 - \frac{ q^{3 - \lambda} } {n} \right)^n
    \\&<&
        \exp{ - q^{3 - \lambda} }
        \ \ \ \ \text{since } 
        \left( 1+\frac{x}{n} \right)^n \leq e^x
    \end{eqnarray*}
    
    Similarly,
    letting $t = \E{X} - \lambda - 1$, we have
    \begin{eqnarray*}
        \Pr{X \geq \E{X} + \lambda}
    &=&
        1 - \Pr{X \leq \E{X} + \lambda - 1}
    \\&=&
        1 - \left( 1 - q^{t + 1} \right)^n
    \\&=&
        1 - \left( 1 - q^{(\E{X} + \lambda - 1) + 1} \right)^n
    \\&=&
        1 - \left( 1 - q^{\E{X} + \lambda } \right)^n
    \\&<&
        1 - \left( 1 - q^{\log_{1/q} n} q^{\lambda} \right)^n
    \\&=&
        1 - \left( 1 - \frac{q^{\lambda}} {n} \right)^n
    \\&<&
        1 - 
        \exp{ - q^{\lambda} } 
        \left( 1 - \frac{ q^{2\lambda} }{n} \right) 
        \ \ \ \ \text{since } 
        e^x \left( 1 - \frac{x^2}{n} \right) 
        \leq \left( 1+\frac{x}{n} \right)^n
    \\&=&
        1 - 
        \exp{ - q^{\lambda} + \ln \left( 1 - \frac{q^{2\lambda}}{n} \right)}
    \\&\leq&
        q^{\lambda} - \ln \left( 1 - \frac{q^{2\lambda}}{n} \right)
        \ \ \ \ \text{since } 1 - e^x \leq - x
    \\&\leq&
        q^{\lambda} + \frac{2 q^{2\lambda}}{n}
        \ \ \ \ \text{since } \ln(1-x) \geq -2x \text{ if } x < 0.7
    \\&\leq&
        q^{\lambda} + q^{2\lambda}
        \ \ \ \ \text{since } n \geq 2.   \qedhere
    \end{eqnarray*}
    % By the union bound,
    % $
    %     \Pr{|X - \E{X}| < \lambda} 
    % < 
    %     \exp{ - q^{3 - \lambda} }
    %     + q^{\lambda}
    %     + q^{2\lambda}.
    % $
\end{proof}




The following corollary for the special case of $p=\frac{1}{2}$ is used for our main result,
showing that a maximum of $\frac{1}{2}$-geometric random variables is 
$\alpha$-$\beta$-sub-exponential for 
$\alpha=4, \beta=\frac{1}{2}$.

\begin{corollary} \label{cor:half-geom-is-sub-exp}
    Let $X_1,\ldots,X_n$ be i.i.d. $\frac{1}{2}$-geometric random variables,
    $n \geq 2$,
    and let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then for all $\lambda > 0$,
    $\Pr{ |X-\E{X}| \geq \lambda } \leq 4 e^{- \lambda / 2}$.
\end{corollary}

\begin{proof}
    By Lemma~\ref{lem:maxGeomTailBound} and the union bound,
    \begin{eqnarray*}
        \Pr{|X - \E{X}| < \lambda}
    &<&
        \exp{ - q^{3 - \lambda} }
        + q^{\lambda} 
        + q^{2\lambda}
    \\&=&
        \exp{ - 2^{\lambda - 3} }
        + 2^{-\lambda} 
        + 2^{-2\lambda}
    \\&<&
        4 e^{-\lambda / 2}.
        \ \ \ \ \text{justified below}
    \end{eqnarray*}
    To see the final inequality,
    differentiate the ratio
    \begin{eqnarray*}
    &&
        \frac{d}{d\lambda}
        \frac
        { \exp{ - 2^{\lambda - 3} }
        + 2^{-\lambda} 
        + 2^{-2\lambda} }
        { 4 e^{-\lambda / 2} }
    \\&=&
        \frac{1}{8}
        \left(
            e^{\lambda/2} 
            \left(
                2^{-2 \lambda} + 2^{-\lambda} 
                + 
                e^{-2^{-3 + \lambda}}
            \right)
        \right)
        + 
        \frac{1}{4}
        \left(
            e^{\lambda/2}
            \left(
                -(
                    2^{1 - 2 \lambda} \ln 2
                ) 
                - \frac
                {\ln 2}
                {2^\lambda} 
                -\frac
                { 2^{-3 + \lambda} \ln 2}
                { e^{2^{-3 + \lambda}} }
            \right)
        \right)
    \end{eqnarray*}
    \todoi{MHS: 
$    
        \exp{ - 2^{\lambda - 3} }
        + 2^{-\lambda} 
        + 2^{-2\lambda}
        <
        2 e^{-\lambda / 2}
        + e^{-\lambda / 2}
        + e^{-\lambda / 2}
        =
        4 e^{-\lambda / 2}
 $ for all $\lambda \geq 1$
    }
    \todo{get a better argument; this is no better than looking at the plot, since I just asked Wolfram Alpha to tell me the derivative and the points where it is 0.}
    This is 0 at $\lambda \approx 1.5$ and $\lambda \approx 1.79$,
    where the ratio is approximately $0.625$.
    Also, at $\lambda=0$ the expression is $< 0.97$,
    and the derivative is negative there.
    Thus, the supremum value of the ratio over all $\lambda \geq 0$
    is $< 0.97$,
    so 
    $
        \exp{ - 2^{\lambda - 3} }
        + 2^{-\lambda} 
        + 2^{-2\lambda}
    <
        4 e^{-\lambda / 2}
    $
    for all $\lambda > 0$.
\end{proof}

% By Corollary~\ref{cor:half-geom-is-sub-exp}
% and Lemma~\ref{lem:subexp-bound-mgf},
% we have the following.

% \begin{corollary} \label{cor:maxGeomSubExp}
%     Let $X_1,\ldots,X_n$ be i.i.d. $\frac{1}{2}$-geometric random variables,
%     let $X = \max\limits_{1 \leq i \leq n} X_i$.
%     Then 
%     for all $|s| \leq \frac{\ln 2}{2}$, 
%     % $\E{e^{s ( X - \E{X} ) } } \leq e^{n s^2 / \ln^2 2}$.
%     we have
%     $\E{e^{s (X - \E{X}) } } , \E{e^{s (\E{X} - X) } } 
%     \leq 1 + 10 s^2 / \ln^2 2$.
% \end{corollary}

\begin{lemma}\label{lem:chernoff-geometric}
    Let $n,K \in \N^+$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then for all $\gamma \geq 0$,
    $\Pr{|X - \E{X}| > \gamma \E{X} } 
    \leq 2 \left( 
            3 n^{- \gamma / 4 }
        \right)^K.$
\end{lemma}

\begin{proof}
    Let $H_n = \sum_{i=1}^n \frac{1}{n}$ be the $n$'th harmonic number,
    recalling that $\ln n < H_n < \ln n + 1$.
    It is known~\cite{eisenberg2008expectation} that 
    $H_n < \E{X_i} < H_n + 1$.
    By linearity of expectation,
    $\E{X} > K H_n > K \ln n$.
    %
    By Corollary~\ref{cor:half-geom-is-sub-exp} 
    and Lemma~\ref{lem:chernoff},
    for $\alpha = 4$ and $\beta = 1/2$,
    we have
    \begin{eqnarray*}
        \Pr{|X - \E{X}| > \gamma \E{X} } 
    &<&
        2
        \frac
        { \left( 1 + \alpha / 2 \right)^K }
        { e^{\gamma \E{X} \beta / 2} }
    <%\\&<&
        2 
        \frac
        { \left( 1 + 4 / 2 \right)^K }
        { e^{\gamma K \ln(n) / 4} }        
    =%\\&=&
        2 
        \left( 
            \frac{3}{n^{\gamma / 4}}
        \right)^K. \qedhere
    \end{eqnarray*}
\end{proof}




\begin{corollary}\label{cor:sumofgeom}
    Let 
    $n \in \N^+$, 
    $\epsilon>0$,
    $C > 2 \epsilon$, 
    $K = C \sqrt{\log n}$, and 
    $n \geq 2^{1 + \left( \frac{C}{C/2-\epsilon} \log 3 \right)^2}$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then
    $$
        \Pr{ \left| \frac{X}{K} - \log n \right| > \frac{1}{2} } 
    \leq 
        \frac{1}{n^\epsilon}.
    $$
\end{corollary}

\todo{this is a little sloppy since I'm assuming $\E{X} = \log n$ exactly, and not taking floors with real numbers.}

\todo{How can we use this to get $\floor{\log n}$? As stated we could compute $\frac{X}{K}$ and round it, but round it the wrong direction and end up with $\floor{\log n} + 1$ or $\floor{\log n} - 1$ instead.}

\begin{proof}
    Let $\gamma = \frac{K}{2 \log n} = \frac{C}{2 \sqrt{\log n}}$.
    Note that $\frac{1}{2} K = \gamma \log n = \gamma \E{X}$.
    %
    Applying Lemma~\ref{lem:chernoff-geometric} with these values of $K$ and $\gamma$,
    \begin{eqnarray*}
        \Pr{ \left| \frac{X}{K} - \log n \right| > \frac{1}{2} } 
    &=&
        \Pr{ \left| X - K \log n \right| > \frac{1}{2} K } 
    \\&=&
        \Pr{ \left| X - \E{X} \right| > \gamma \E{X} } 
    \\&\leq&
        2
        \left( 
            3 n^{- \gamma / 4}
        \right)^K
    \\&=&
        2
        \left( 
            3 n^{- \frac{C}{2 \sqrt{\log n} } }
        \right)^{C \sqrt{\log n}}
    \\&<& 
        2 \cdot
        3^{C \sqrt{\log n} } n^{-C/2}.
    \end{eqnarray*}
    
    We claim that this quantity is at most 
    $\frac{1}{n}$ for sufficiently large $n$.
    To see why, we show that 
    for any $C > 2\epsilon$,
    $2 \cdot 3^{C \sqrt{\log n}} \leq n^{C/2-\epsilon}$
    for all sufficiently large $n$.
    Taking logs of both sides,
    \begin{eqnarray*}
        2 \cdot 3^{C \sqrt{\log n}} \leq n^{C/2-\epsilon}
    &\iff&
        \log(2) + C \sqrt{\log n} \log 3 \leq (C/2-\epsilon) \log n
    \\&\iff&
        1 + \frac{C}{C/2-\epsilon} \log 3 \leq \sqrt{\log n}
    \\&\iff&
        2^{1 + \left( \frac{C}{C/2-\epsilon} \log 3 \right)^2} \leq n,
    \end{eqnarray*}
    Thus,
    $\Pr{ \left| \frac{X}{K} - \log n \right| > \frac{1}{2} } < \frac{1}{n^\epsilon}.$
\end{proof}

For example, for $C=12$ and $\epsilon=1$
(for probability of error at most $\frac{1}{n}$), 
it suffices to have $n \geq 45379$.
If we let $\epsilon \to 0$,
the lower bound on $n$ approaches $2^{1 + (2 \log 3)^2} \approx 2117$.

\todoi{
    Is there a way to cut down on the memory requirements? 
    The naive implementation stores all $K=C \sqrt{\log n}$ variables, 
    which each will mostly end up close to $\log n$, each requiring $\log \log n$ bits, 
    but this means we need $K \log \log n$ bits, or $\log^{K} n$ states, 
    which is quite a lot 
    (it's smaller than $n^\epsilon$ for any $\epsilon$, but still much more than polylog$(n)$). 
    Can we be more clever and not have to remember the exact value of all of them?
}
\todoi{MHS: For cutting down the space usage we can store the difference of each number and the tuple size. Each time the tuple size increases we also have to update numbers agent stores. (positive and negative difference is needed) In this way we save a constant factor of $\log \log n$ bits which would be a constant factor in the power of $\log^K n $ states}
\todoi{State a separate corollary for estimating $\floor{ \log \log n}$, which is all that is needed for the $\log \log n$-state leader election. It will still use more memory, but won't need as much as in the case of getting $\floor{\log n}$ exactly. We only need to get $\log n$ within factor 2, so $K$ can be much smaller (hopefully something like $\log \sqrt{\log n}$ or something.}




==> sections/old/stronger-geometric.tex <==
\subsection{Chernoff bound on sums of maxima of geometric random variables}
\label{subsec:geom}

% \todoi{
%     Looking into ``subexponential'' random variables for possibly proving tail inequalities on maximums of geometric random variables: 
    
%     \url{https://www.stat.berkeley.edu/~mjwain/stat210b/Chap2_TailBounds_Jan22_2015.pdf}
    
%     \url{http://tinyurl.com/y8r772hv}
    
%     This paper shows that geometric r.v.'s are sub-exponential: 
%     \url{https://arxiv.org/pdf/1301.3321.pdf}
    
%     This shows how to bound the maximum of sub-gaussian; perhaps we can imitate the proof for sub-exponential: 
%     \url{https://ocw.mit.edu/courses/mathematics/18-s997-high-dimensional-statistics-spring-2015/lecture-notes/MIT18_S997S15_Chapter1.pdf}
% }

\subsubsection{Sub-exponential random variables}

\begin{definition}
    Let $\alpha,\beta > 0$ and let $X$ be a random variable.
    We say $X$ is \emph{$\alpha$-$\beta$-sub-exponential} if,
    for all $\lambda>0$,
    $\Pr{X \geq \lambda} \leq \alpha e^{-\beta \lambda}$.
\end{definition}

The following lemma is well-known;
we prove it explicitly since its exact form differs from common bounds in the literature.
It shows that exponential tail bounds $\Pr{|X-\E{X}| > \lambda}$ on a random variable $X$ give bounds on the moment-generating functions of the random variables $X-\E{X}$ and $\E{X}-X$.
The proof is modeled on Rigollet's proof of the analogous lemma for sub-gaussian random variables proven in~\cite{rigollet2015highdimensional}.

\todo{See if there's a way to avoid this ugliness with having two separate bounds. It's here because of the problem Eric pointed out, where $\E{X-\E{X}} = \E{\E{X}-X} = 0$, but $\E{|X-\E{X}|} \neq 0$.}

\begin{lemma}[\cite{rigollet2015highdimensional}] \label{lem:subexp-bound-mgf}
    Let $X$ be an $\alpha$-$\beta$-sub-exponential random variable.
    Then for all $s \in [-\beta/2, \beta/2]$, 
    we have
    $\E{ e^{ s (X-\E{X}) } } , \E{ e^{ s (\E{X}-X) } } 
    \leq 1 + 2 \alpha s^2 / \beta^2$.
\end{lemma}

\begin{proof}
    Let $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{|X - \E{X}|^k}
    &=&
        \int_0^\infty \Pr{|X - \E{X}|^k \geq \lambda} d\lambda
    =%\\&=&
        \int_0^\infty \Pr{|X - \E{X}| \geq \lambda^{1/k}} d\lambda
    \\&\leq&
        \int_0^\infty \alpha e^{-\beta \lambda^{1/k}} d\lambda
    =%\\&=&
        \alpha \frac{1}{\beta^k} k \int_0^\infty e^{-u} u^{k-1} du  
        \ \ \ \ \ \ \text{substituting } u = \beta \lambda^{1/k}
    \\&=&
        \frac{\alpha}{\beta^k} k \Gamma(k)
    =
        \frac{\alpha}{\beta^k} k!,
    \end{eqnarray*}
    where $\Gamma(k)$ is the \emph{gamma function} 
    (defined by the given integral),
    known to equal $(k-1)!$ for $k \in \N^+$.
    Then
    \begin{eqnarray*}
        \E{e^{s (X - \E{X}) }}
    &=&
        \E{ \sum_{k=0}^\infty 
        \frac{ ( s (X - \E{X}) )^k }{k!} } 
        \ \ \ \ \ \text{Taylor expansion of the exponential function}
    \\&=&
        \sum_{k=0}^\infty 
        \frac{ s^k \E{(X - \E{X})^k} }{k!} 
        \ \ \ \ \ \ \ \text{dominated convergence theorem}
    \\&=&
        1 + 
        s \underbrace{ \E{X - \E{X}} }_{= 0} + 
        \sum_{k=2}^\infty 
        \frac{ s^k \E{(X - \E{X})^k} }{k!}
    \\&\leq&
        1 + 
        \sum_{k=2}^\infty 
        \frac{ |s|^k \E{|X - \E{X}|^k} }{k!}
        \ \ \ \text{odd terms can only get larger}
    \\&\leq&
        1 + 
        \sum_{k=2}^\infty 
        \frac{ |s|^k \frac{\alpha}{\beta^k} k! }{k!}
    =%\\&=&
        1 + 
        \alpha 
        \sum_{k=2}^\infty 
        \left( \frac{|s|}{\beta} \right)^k
    =%\\&=&
        1 + 
        \alpha \frac{s^2}{\beta^2} 
        \sum_{k=0}^\infty 
        \left( \frac{|s|}{\beta} \right)^k
    % \\&=&
    %     1 + 
    %     \alpha \frac{s^2}{\beta^2} 
    %     \frac{1}{1 - |s|/\beta}
    \\&\leq&
        1 + \alpha \frac{s^2}{\beta^2} \sum_{k=0}^\infty \frac{1}{2^k} 
        \ \ \ \ \ \ \ \ \ \ \ \text{since $|s| \leq \frac{\beta}{2}$}
    \\&=&
        1 + 2 \alpha \frac{s^2}{\beta^2} .
    \end{eqnarray*}
    The bound for $\E{ e^{ s (\E{X}-X) } }$
    is derived by a similar argument.
\end{proof}






The following Chernoff bound is similarly well-known,
but stated in a more convenient form for our purposes.

\begin{lemma}\label{lem:chernoff}
    Let $\alpha,\beta > 0$ and $K \in \N^+$.
    Let $X_1,\ldots,X_K$ be i.i.d. $\alpha$-$\beta$-sub-exponential random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then for all $t \geq 0$,
    $$
        \Pr{|X - \E{X}| \geq t } 
    \leq
        2
        \frac
        { \left( 1 + \alpha / 2 \right)^K }
        { e^{t \beta / 2} }.
    $$
\end{lemma}

\begin{proof}
    Then for all $t>0$,
    \begin{eqnarray*}
        \Pr{X - \E{X} \geq t}
    &=& 
        \Pr{e^{ s (X - \E{X}) } \geq e^{s t}} 
    \\&\leq& 
        \frac
        { \E{e^{s (X - \E{X}) } } } 
        { e^{s t} } 
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{Markov's inequality}
    \\&=&
        e^{- s t} 
        \E{ e^{ s \left( \left( \sum_{i=1}^K X_i \right) - \E{X} \right) } }
    \\&=&
        e^{- s t} 
        \E{ e^{ s \sum_{i=1}^K ( X_i  - \E{X_i} ) } }
        \ \ \ \ \text{linearity of expectation}
    \\&=& 
        e^{- s t} 
        \E{ \prod_{i=1}^K e^{s ( X_i - \E{X_i} ) } } 
    \\&=& 
        e^{- s t} 
        \prod_{i=1}^K 
        \E{ e^{s ( X_i - \E{X_i} ) } }. 
        \ \ \ \ \text{independence of the $X_i$'s}
    \end{eqnarray*}
    
    By Lemma~\ref{lem:subexp-bound-mgf},
    for all $|s| \leq \frac{\beta}{2}$,
    $\E{ e^{s (X_i - \E{X_i}) } } \leq 1 + 2 \alpha s^2 / \beta^2$.
    So
    $
        \Pr{X - \E{X} \geq t} 
    \leq 
        e^{- s t }
        (1 + 2 \alpha s^2 / \beta^2)^K.
    $
    %
    Let $s = \frac{\beta}{2}$. 
    Then
    $
    \Pr{ X - \E{X} \geq t }
    \leq e^{- s t}
        \left( 1 + 2 \alpha s^2 / \beta^2 \right)^K
    = e^{- t \beta / 2}
        \left( 1 + \alpha / 2 \right)^K.
    $
    % \begin{eqnarray*}
    %     \Pr{ X - \E{X} \geq t }
    % \leq %&\leq&
    %     e^{- s t}
    %     \left( 1 + 2 \alpha s^2 / \beta^2 \right)^K
    % =%\\&=&
    %     e^{- t \beta / 2}
    %     \left( 1 + \alpha / 2 \right)^K.
    % % \\&=&
    % %     e^{- \gamma \E{X} \beta / 2}
    % %     \left( 1 + \frac{ K \alpha / 4} {K} \right)^K
    % % \\&<&
    % %     e^{- \gamma \E{X} \beta / 2}
    % %     e^{- K \alpha / 4 }
    % % \\&<&
    % %     e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }
    % \end{eqnarray*}
    The proof that 
    $
        \Pr{\E{X} - X \geq t} 
        % < e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }
        <
        e^{- t \beta / 2}
        \left( 1 + \alpha / 2 \right)^K
    $
    is symmetric.
    By the union bound,
    $
        \Pr{|X-\E{X}| \geq t} 
    < 
        % 2 e^{- \gamma \E{X} \beta / 2 - K \alpha / 4 }.
        2 e^{- t \beta / 2}
        \left( 1 + \alpha / 2 \right)^K.
    $
\end{proof}
























\subsubsection{Geometric random variables and their maximum}

We say $X$ is a \emph{$p$-geometric random variable}
if it is the number of consecutive $T$'s before the first $H$,
when flipping a coin with $\Pr{H}=p$
(\emph{not} counting the flip that results in the first $H$).
Thus $\E{X} = \frac{1}{p} - 1$;
in particular $\E{X} = 1$ if $p = \frac{1}{2}$.

The next lemma shows a tail bound on a maximum of geometric random variables.

\todoi{DD: see if we can change $q^{3 - \lambda}$ to $q^{2 - \lambda}$ by substituting $\Pr{|X-\E{X}| > \lambda}$ for $\Pr{|X-\E{X}| \geq \lambda}$. It seems okay to do as long as we track it through the proof of the sub-exponential lemma, but it seems strange to do since these are integer-valued random variables and it seems cleanest to use $\geq$}

\begin{lemma} \label{lem:maxGeomTailBound}
    Let $p=\frac{1}{2}$.
    Let $X_1,\ldots,X_n$ be i.i.d. $p$-geometric random variables,
    $n \geq 2$,
    let $q=1-p=\frac{1}{2}$,
    and let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then for all $\lambda > 0$,
    $
        \Pr{ \E{X}-X \geq \lambda } 
    \leq 
        \exp{ - q^{1 - \ln q - \lambda} }
    $
    and
    $
        \Pr{ X-\E{X} \geq \lambda } 
    \leq 
        q^{\lambda-1} + q^{2\lambda-2}.
    $
\end{lemma}

\begin{proof}
    For each $t \in \N$, 
    $
        \Pr{X_i \geq t}
        = q^{t}
    $,
    so
    $
        \Pr{X_i \leq t}
        = 1 - \Pr{X_i \geq t+1}
        = 1 - q^{t+1}.
    $
    
    Since the $X_i$'s are independent,
    $
        \Pr{X \leq t} 
        = \prod_{i=1}^n \left( 1 - q^{t+1} \right)
        = \left( 1 - q^{t+1} \right)^n.
    $
    
    Let $H_n = \sum_{i=1}^n \frac{1}{n}$ be the $n$'th harmonic number,
    recalling that $\ln n < H_n < \ln n + 1$.
    For $n \geq 22$,
    $H_n - \ln n - 0.577 \leq 0.024$,
    so 
    $H_n \leq \ln n + 0.56$,
    and for $n \geq 22$,
    $H_n \geq \ln n + 0.6$.
    It is known~\cite{eisenberg2008expectation} that 
    $\frac{1}{\lambda} H_n - 1 \leq \E{X} < \frac{1}{\lambda} H_n$,\footnote{
        Eisenberg~\cite{eisenberg2008expectation} studies the variant of a geometric random variable that counts the first heads, which is 1 greater than our variant.
        To compensate we subtract 1 from the bounds on $\E{X}$ stated in~\cite{eisenberg2008expectation}.
    }
    where $q = e^{-\lambda}$,
    i.e. $\lambda = \ln(1/q)$.
    Eisenberg shows a stronger result,
    that for $q \geq 0.368$ and $n \geq 10$,
    $\left| \E{X} - \left( \frac{1}{\ln(1/q)} H_n - \frac{1}{2} \right) \right| < 0.0006$.
    
    For $q=\frac{1}{2}$,
    
    Combining these,
    we have that for $q=\frac{1}{2}$,
    $\E{X} 
    < 0.0006 + \left( \frac{1}{\ln 2} H_n - \frac{1}{2} \right)
    \leq 0.0006 + \frac{1}{\ln 2} (\ln n + 0.532) - \frac{1}{2}
    = 0.0006 + \log_2 n + \frac{0.53}{\ln 2} - \frac{1}{2}
    < \log_2 n + 0.27$
    and
    $\E{X} 
    > - 0.0006 + \left( \frac{1}{\ln 2} H_n - \frac{1}{2} \right)
    \geq - 0.0006 + \frac{1}{\ln 2} (\ln n + 0.53) - \frac{1}{2}
    = - 0.0006 + \log_2 n + \frac{0.53}{\ln 2} - \frac{1}{2}
    < \log_2 n + 0.27$
    
    Thus
    $\frac{1}{\ln(1/q)} \ln n - 1 < \E{X} < \frac{1}{\ln(1/q)} (\ln n + 1)$,
    i.e.,
    $\log_{1/q} n - 1< \E{X} < \log_{1/q} n - \ln q$.
    %\todo{The second inequality here is not correct. It is more like $\E{X} < \log_{1/q} n + 1 + \ln \frac{1}{q}$, which can get large for $q$ close to 0. It is correct for $q=1/2$, since $\ln \frac{1}{q} \approx 0.693$}
    %$\log_{1/q} n < \E{X} < \log_{1/q} n + 2$.
    %\todoi{MHS: The todo on the right side seems wrong, because the second inequality would be like $\E{X} < \log_{1/q} n + 1 + \frac{1}{\ln \frac{1}{q}}$. So, even for $q=1/2$ it is more than $2$.}
% Got the next bound from here:
% Or we could just use this: \url{http://www.lkozma.net/inequalities_cheat_sheet/ineq.pdf}
% which states $(1+\frac{x}{n})^n \geq e^x (1 - \frac{x^2}{n})$.
% See also \url{https://math.stackexchange.com/questions/259543/rate-of-convergence-of-left1-fracax-rightx-to-operatornameexpa}

    Below we use the inequalities
    $e^x \left( 1 - \frac{x^2}{n} \right) 
    \leq \left( 1+\frac{x}{n} \right)^n 
    \leq e^x$
    for $n > 1, |x| < n$.

    Setting $t = \E{X} - \lambda$, we have
    \begin{eqnarray*}
        \Pr{X \leq \E{X} - \lambda}
    &=&
        \left( 1 - q^{t + 1} \right)^n
    \\&=&
        \left( 1 - q^{(\E{X} - \lambda) + 1} \right)^n
    \\&<&
        \left( 1 - q^{\log_{1/q} n - \ln q - \lambda + 1} \right)^n
    \\&=&
        \left( 1 - q^{\log_{1/q} n} q^{1 - \ln q - \lambda} \right)^n
    \\&=&
        \left( 1 - \frac{ q^{1 - \ln q - \lambda} } {n} \right)^n
    \\&<&
        \exp{ - q^{1 - \ln q - \lambda} }
        \ \ \ \ \text{since } 
        \left( 1+\frac{x}{n} \right)^n \leq e^x
    \end{eqnarray*}
    
    Similarly,
    letting $t = \E{X} + \lambda - 1$, we have
    \begin{eqnarray*}
        \Pr{X \geq \E{X} + \lambda}
    &=&
        1 - \Pr{X \leq \E{X} + \lambda - 1}
    \\&=&
        1 - \left( 1 - q^{t + 1} \right)^n
    \\&=&
        1 - \left( 1 - q^{(\E{X} + \lambda - 1) + 1} \right)^n
    \\&=&
        1 - \left( 1 - q^{\E{X} + \lambda } \right)^n
    \\&<&
        1 - \left( 1 - q^{\log_{1/q} n - 1 + \lambda} \right)^n
    \\&=&
        1 - \left( 1 - q^{\log_{1/q} n} q^{\lambda-1} \right)^n
    \\&=&
        1 - \left( 1 - \frac{q^{\lambda-1}} {n} \right)^n
    \\&<&
        1 - 
        \exp{ - q^{\lambda-1} } 
        \left( 1 - \frac{ q^{2(\lambda-1)} }{n} \right) 
        \ \ \ \ \text{since } 
        e^x \left( 1 - \frac{x^2}{n} \right) 
        \leq \left( 1+\frac{x}{n} \right)^n
    \\&=&
        1 - 
        \exp{ - q^{\lambda-1} + \ln \left( 1 - \frac{q^{2\lambda-2)}}{n} \right)}
    \\&\leq&
        q^{\lambda-1} - \ln \left( 1 - \frac{q^{2\lambda-2}}{n} \right)
        \ \ \ \ \text{since } 1 - e^x \leq - x
    \\&\leq&
        q^{\lambda-1} + \frac{2 q^{2\lambda-2}}{n}
        \ \ \ \ \text{since } \ln(1-x) \geq -2x \text{ if } x < 0.7
    \\&\leq&
        q^{\lambda-1} + q^{2\lambda-2}
        \ \ \ \ \text{since } n \geq 2.   \qedhere
    \end{eqnarray*}
\end{proof}




The following corollary for the special case of $p=\frac{1}{2}$ is used for our main result,
showing that a maximum of $\frac{1}{2}$-geometric random variables is 
$\alpha$-$\beta$-sub-exponential for 
$\alpha=7, \beta=\frac{1}{2}$.

\begin{corollary} \label{cor:half-geom-is-sub-exp}
    Let $X_1,\ldots,X_n$ be i.i.d. $\frac{1}{2}$-geometric random variables,
    $n \geq 2$,
    and let $X = \max\limits_{1 \leq i \leq n} X_i$.
    Then for all $\lambda > 0$,
    $\Pr{ |X-\E{X}| \geq \lambda } \leq 7 e^{- \lambda / 2}$.
\end{corollary}

\begin{proof}
    By Lemma~\ref{lem:maxGeomTailBound} and the union bound,
    \begin{eqnarray*}
        \Pr{|X - \E{X}| < \lambda}
    &<&
        \exp{ - q^{1 - \ln q - \lambda} }
        + q^{\lambda-1} 
        + q^{2\lambda-2}
    \\&=&
        \exp{ - 2^{\lambda - \ln 2} }
        + 2^{1-\lambda} 
        + 2^{2-2\lambda}
    \\&<&
        7 e^{-\lambda / 2}.
        \ \ \ \ \text{justified below}
    \end{eqnarray*}
    To see the final inequality,
    differentiate the ratio
    \begin{eqnarray*}
    &&
        \frac{d}{d\lambda}
        \frac
        { \exp{ - 2^{\lambda - 1 - \ln 2} }
        + 2^{-\lambda} 
        + 2^{-2\lambda} }
        { 7 e^{-\lambda / 2} }
    \\&=&
        \frac{1}{14}
        \left(
            e^{\lambda/2} 
            \left(
                2^{-2 \lambda} + 2^{-\lambda} 
                + 
                e^{-2^{\lambda - 1 - \ln 2}}
            \right)
        \right)
        + 
        \frac{1}{7}
        \left(
            e^{\lambda/2}
            \left(
                -(
                    2^{1 - 2 \lambda} \ln 2
                ) 
                - \frac
                {\ln 2}
                {2^\lambda} 
                -\frac
                { 2^{\lambda - 1 - \ln 2} \ln 2}
                { e^{2^{\lambda - 1 - \ln 2}} }
            \right)
        \right)
    \end{eqnarray*}
    \todoi{MHS: 
$    
        \exp{ - 2^{\lambda - 3} }
        + 2^{-\lambda} 
        + 2^{-2\lambda}
        <
        2 e^{-\lambda / 2}
        + e^{-\lambda / 2}
        + e^{-\lambda / 2}
        =
        4 e^{-\lambda / 2}
 $ for all $\lambda \geq 1$
 DD: why?
    }
    \todo{get a better argument; this is no better than looking at the plot, since I just asked Wolfram Alpha to tell me the derivative and the points where it is 0.}
    This expression is $<0$ for $\lambda \geq 0$
    and at $\lambda=0$ the expression is $< 0.97$,
    and the derivative is negative there.
    Thus, the supremum value of the ratio over all $\lambda \geq 0$
    is $< 0.97$,
    so 
    $
        \exp{ - 2^{\lambda - 3} }
        + 2^{-\lambda} 
        + 2^{-2\lambda}
    <
        7 e^{-\lambda / 2}
    $
    for all $\lambda > 0$.
\end{proof}

% By Corollary~\ref{cor:half-geom-is-sub-exp}
% and Lemma~\ref{lem:subexp-bound-mgf},
% we have the following.

% \begin{corollary} \label{cor:maxGeomSubExp}
%     Let $X_1,\ldots,X_n$ be i.i.d. $\frac{1}{2}$-geometric random variables,
%     let $X = \max\limits_{1 \leq i \leq n} X_i$.
%     Then 
%     for all $|s| \leq \frac{\ln 2}{2}$, 
%     % $\E{e^{s ( X - \E{X} ) } } \leq e^{n s^2 / \ln^2 2}$.
%     we have
%     $\E{e^{s (X - \E{X}) } } , \E{e^{s (\E{X} - X) } } 
%     \leq 1 + 10 s^2 / \ln^2 2$.
% \end{corollary}

\begin{lemma}\label{lem:chernoff-geometric}
    Let $n,K \in \N^+$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then for all $t \geq 0$,
    $\Pr{|X - \E{X}| \geq t } 
    \leq 2 \cdot  e^{K \ln(9/2) - t/4}.$
\end{lemma}

\begin{proof}
    Let $H_n = \sum_{i=1}^n \frac{1}{n}$ be the $n$'th harmonic number,
    recalling that $\ln n < H_n < \ln n + 1$.
    It is known~\cite{eisenberg2008expectation} that 
    $H_n < \E{X_i} < H_n + 1$.
    By linearity of expectation,
    $\E{X} > K H_n > K \ln n$.
    %
    By Corollary~\ref{cor:half-geom-is-sub-exp} 
    and Lemma~\ref{lem:chernoff},
    for $\alpha = 7$ and $\beta = 1/2$,
    we have
    \begin{eqnarray*}
        \Pr{|X - \E{X}| > t } 
    &<&
        2
        \frac
        { \left( 1 + \alpha / 2 \right)^K }
        { e^{t \beta / 2} }
    <%\\&<&
        2 
        \frac
        { \left( 9 / 2 \right)^K }
        { e^{t / 4} } 
    =%\\&=&
        2 \cdot  (9/2)^K \cdot  e^{-t/4}
    =%\\&=&
        2 \cdot  e^{K \ln(9/2) - t/4}. \qedhere
    \end{eqnarray*}
\end{proof}




\begin{corollary}\label{cor:sumofgeom}
    Let 
    $a > 4\ln(9/2) \approx 6$,
    $n \in \N^+$, 
    %$\epsilon>0$,
    %$C > 2 \epsilon$, 
    $K \geq \frac{\ln n}{a/4 - \ln(9/2)}$. %, and 
    %$n \geq 2^{1 + \left( \frac{C}{C/2-\epsilon} \log 3 \right)^2}$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then
    $$
        \Pr{ \left| \frac{X}{K} - \log n \right| \geq a } 
    \leq 
        \frac{2}{n}.
    $$
\end{corollary}

\todo{this is a little sloppy since I'm assuming $\E{X} = \log n$ exactly, and not taking floors with real numbers.}

\todo{How can we use this to get $\floor{\log n}$? As stated we could compute $\frac{X}{K}$ and round it, but round it the wrong direction and end up with $\floor{\log n} + 1$ or $\floor{\log n} - 1$ instead.}

\begin{proof}
    Let $t = aK$.
    Applying Lemma~\ref{lem:chernoff-geometric} with these values of $K$ and $t$,
    \begin{eqnarray*}
        \Pr{ \left| \frac{X}{K} - \log n \right| > a } 
    &=&
        \Pr{ \left| X - K \log n \right| > aK } 
    \\&=&
        \Pr{ \left| X - \E{X} \right| > t } 
    \\&\leq&
        2 \cdot  e^{K \ln(9/2) - t/4}
    \\&=&
        2 \cdot  e^{K (\ln(9/2) - a/4)}
    \\&=&
        2 \cdot  e^{- K (a/4 - \ln(9/2))}
    \\&\leq&
        2 \cdot  e^{- \frac{\ln n}{a/4 - \ln(9/2)} (a/4 - \ln(9/2)) }
    \\&=& 
        2 \cdot  e^{- \ln n}
    \\&=& 
        \frac{2}{n}. \qedhere
    \end{eqnarray*}
\end{proof}

For example,
choosing $a = 4 (\ln 2 + \ln(9/2)) < 8.8$ means we can choose
$K 
\geq \frac{\ln n}{a/4 - \ln(9/2)} 
= \frac{\ln n}{4(\ln 2 + \ln(9/2))/4 - \ln(9/2)} 
= \frac{\ln n}{\ln 2}
= \log_2 n$:

\begin{corollary}\label{cor:sumofgeomConcreteK}
    Let 
    $n \in \N^+$, 
    %$\epsilon>0$,
    %$C > 2 \epsilon$, 
    $K = \ceil{\log n}$. %, and 
    %$n \geq 2^{1 + \left( \frac{C}{C/2-\epsilon} \log 3 \right)^2}$.
    Let $X_1,\ldots,X_K$ be i.i.d. random variables,
    each of which is the maximum of $n$ i.i.d. $\frac{1}{2}$-geometric random variables.
    Define $X = \sum_{i=1}^K X_i$.
    Then
    $$
        \Pr{ \left| \frac{X}{K} - \log n \right| \geq 8.8 } 
    \leq 
        \frac{2}{n}.
    $$
\end{corollary}





==> sections/protocol-subsec-det.tex <==
%\subsection{The protocol}

\subsection{Intuition}
Alistarh et al.~\cite{alistarh2017time} describe a protocol for estimating $\log n$ 
within a constant multiplicative factor. 
%\dds{Where a}
%\todo{Alter all geometric r.v.s to count the success so they have a consistent definition throughout the paper.}
A $\frac{1}{2}$-geometric random variable is the number of flips needed to get one head when flipping a fair coin. 
In their protocol, each agent generates an independent geometric random variable $\mathbf{G}_i$,
then propagates the maximum 
$\mathbf{M} = \max_{1 \leq i \leq n} \mathbf{G}_i$
by \emph{epidemic}:
transitions of the form $i,j \to j,j$ for $i \leq j$, 
which in $O(\log n)$ time ``infect'' all agents with the maximum.
It is known that $\E{\mathbf{M}} \approx \log n$~\cite{eisenberg2008expectation},
and $\log n - \log \ln n \leq \mathbf{M} \leq 2 \log n$ with probability 
$\geq 1-O(1)/n$ (Lemma~\ref{cor:half-geom-tighter-bounds}). 

% \dds{
%     Here, we are going to use the idea of propagating the maximum of $n$ i.i.d geometric random variable with repetition.
%     Let's assume each agent instead of $1$ random variable carries a tuple of $K$ random variables. 
%     Then, they would propagate the pointwise maximum by the epidemic. Setting $K=4{\log n}$
%     will give us an additive error with high probability \ref{cor:sumofgeom}. Though, if all agents were supposed to carry all the generated random numbers, the number of states would grow from $O(\log n)$ to $O(\log^{\log n} n)$. In the following protocol, we are going to perform the $K$ independent round with having each agent carry only a constant number of random variable. Intuitively, each agent is responsible for propagating one index (called $\indx$) of the tuple out of $K$ possible Indices. Setting $K=O(\log n)$ would roughly mean $O(\frac{n}{\log n})$ agents are responsible for propagating each index.
% }{}

We take the obvious extension of this approach:
do this $K$ times and take an average.
The estimated average is within $O(1)$ of $\log n$ so long as $K = \Omega(\log n)$
(Corollary~\ref{cor:sumofgeomConcreteK}).
One problem to solve first is how to calculate $K$;
after all, $K = \Theta(\log n)$ scales with $n$,
so with a uniform protocol it cannot be encoded into the agents at the start.
The agents estimate it using the protocol of~\cite{alistarh2017time}.
% Furthermore,
% our analysis in Subsection~\ref{subsec:geom} gives tighter bounds than $\frac{1}{2} \log n$ and $9 \log n$ from~\cite{alistarh2017time}.
% This estimate is used to calculate $K$.
Since that protocol is converging but not terminating
(provably it cannot be made terminating by Theorem~\ref{thm:main-termination}),
each time an agent updates its value of $K$,
it reinitializes the remainder of its state.

However, a trickier problem remains: 
a na\"{i}ve approach to implement ``averaging of $K$ numbers'' requires storing $K = \Theta(\log n)$ numbers in each agent,
each having value $\Theta(\log n)$,
implying the number of states is $\Theta((\log n)^{\log n}) = \Theta(n^{\log \log n})$.
This is even more than the $O(n^{60})$ sufficient to quickly compute \emph{exactly} $n$~\cite{doty2018exact}.
% In a population with an existing unique leader, we can design a timer that goes off after the maximum generated one is propagated with high probability. The leader is responsible for simulating the timer and keeps track of $K$ sequential calls to a subprotocols for generating one geometric random variable and propagating the maximum amongst the population via epidemic. The leader is responsible to reset the timer and call the subprotocol again until $K$ calls have been done. At each round, agents will generate a new random variable and propagate the maximum amongst until the leader signals through the population to move to the next round, then they store the current random variable to their sum field and start over.
% The above idea will work properly in a population with a leader. Although we assume our population doesn't have a unique leader to set the timer. We overcome this obstacle by designing a leaderless phase clock inside each agent. 
To overcome this problem, we use a ``leaderless phase clock'':
a leaderless phase clock similar to those of~\cite{alistarh2018space,sudo2018logarithmic,mocquard2018population} but uniform.
Unlike the phase clock used 
by~\cite{alistarh2018space,mocquard2018population}, our presented leaderless phase clock utilize one simple rule for all the agents to increase their counter on every interaction. 
This simultaneously gives an elegant way to compose our protocols with downstream protocols requiring the size estimate.
Agents count their number of interactions and compare it with a threshold value $\Theta(\log n)$.
Whenever their number of interaction passes the threshold they will move to the next round similar to the protocol described above (the population with a leader). 
The threshold is calculated in the following way.
In our protocol, agents start generate a geometric random variable called \clock\ and propagate the maximum \clock\ among themselves. 
After agents agree on the $\clock$ variable, a constant multiple $\cte . \clock$ is the threshold in their leaderless phase clock.
This lets the agents synchronize epochs of the algorithm,
each taking $O(\log n)$ time,
and prevent the next epoch from starting until the previous has concluded.

The probabilistic clock inside agents might go off very soon at the very beginning of the protocol, 
but after $O(\log n)$ time all agents will store the maximum generated \clock\ and their leaderless phase clock will eventually converge to a stable one which goes off after completion of a predefined constant factor of $\log n$;
to handle this, each time an agent updates its value of $\clock$,
the remainder of its state is reset and it begins the rest of the protocol anew.
Restarting the downstream protocol is a known technique in population protocols also used in~\cite{GS18} to compose two leader elimination protocols.
The agents then generate $K$ additional geometric random variables in sequence, taking their sum. 
% agents wait $\cte . \clock$ time to make sure all agents are at the same step of the protocol and all of them got the maximum value of the corresponding \phase\ by epidemic. 
Upon completing the generation and propagation of the $K$'th number, 
the agent divides the sum by $K$ and stores the result in their output field.
Composition with a downstream protocol is as simple as letting that protocol be the last phase.
However, since our protocol has a positive probability of failure, 
this would translate to the downstream protocol as well.

The time is $O(\log^\timeExponent n)$ by the following rough analysis
(details follow).
We propagate $K$ numbers one after each other and for each epidemic $O(\log n)$ time is required. Since we set $k = O(\log n)$ then the protocol will take $O(\log^2 n)$ total time to complete.



\opt{sub}{\vspace{-0.2cm}}
\subsection{Formal specification of protocol} 
\label{subsec:protocol}


%\todoi{instead of multiplying $\init$ by $c_\text{init}$, add $\log \ln \init$ to it (or something similar) since we can prove that $\init$ is likely to be at least $\log n - \log \ln n$.}
Our protocol uses uniform random bits in multiple places. 
We use the inherent randomness of the uniform random scheduler to simulate our own random bits  similar to that of~\cite{sudo2018logarithmic}. 
In the protocol, agents start by dividing in two groups of \f\ and \a. \a\ agents are responsible to compute the algorithm while the \f\ agents only provide fair coin flips. 
When an \a\ agent interact with an \f\ agent, 
with probability exactly $\frac{1}{2}$ each can be the sender or the receiver;
this is used to assign the random bit to the $\a$ agent.

%They have a ``role'' field, initially \x\ for ``no role''. If two agents in role \x\ interact with each other the sender changes its role to \a\ (algorithm) and the receiver changes its role to \f (``coin flip''). If we restrict ourselves to this rule, exactly half of the agents become \a\ and half of them become \f\ eventually. However, this protocol takes linear time for all agents to change their role for \x\ to either \a\ of \f. 
Agents initially have no role ($\x$),
and partition into roles via $\x,\x \to \a,\f$.
Since this takes $\Theta(n)$ time to complete,
we add transitions $\a,\x \to \a,\f$ and $\f,\x \to \f,\a$,
converging in $O(\log n)$ time, 
with the price of deviating from $\frac{n}{2}$ for each role. 
By Lemma~\ref{lem:boundOnCardinalityOfA} this deviation is $O(\sqrt{n \ln n})$,
increasing the size estimation error by merely a constant additive factor.\footnote{
    This mechanism of splitting the population approximately in two works for our protocol,
    because the number of $\a$ agents is likely to be so close to $n/2$ that our estimate of $\log n$ is reduced by an additive factor likely to be very close to $-1$.
    If some downstream protocol requires all agents to participate in the algorithm
    (e.g., for predicate computation),
    then a similar but more complex scheme works instead:
    All agents count their number of interactions mod 2,
    acting in the $\a$ role on even interactions and the $\f$ role on odd interactions.
    This implies a similar constant-factor slowdown,
    and it obtains the required independence of coin flips from each other and from algorithm steps.
}

All agents start at $\phase =0$. 
%The agents in the \a\ role are responsible for running the protocol and computing an estimation of $\log n$ while the agents in the \f\ role are only responsible for generating random bits. Whenever two agents in different roles (\a\ and \f) interact with each other the agent in the \a\ role can use the inherent randomness of the scheduler and generate one random bit based on its role (receiver or sender) in that interaction. Since the agent can be sender with probability exactly $\frac{1}{2}$ and receiver with probability $\frac{1}{2}$ the generated random bit is fair.
% They use each random bit once and generate a new one in their future interactions. 
The $\a$ agent use random bits,
obtained by a synthetic coin technique 
(due to~\cite{sudo2018logarithmic}) 
through interaction with $\f$ agents,
to generate a geometric random variable. 
In protocol~\ref{subprotocol:genClk} an \a\ agent starts with $1$ in its \clock\ field and increases it as long as it is the sender (``coin flip = tails'') 
in an interaction with an \f\ agent. 
When an \a\ agent interacts as the receiver (``coin flip = heads'') with an \f\ agent, 
it will set a flag meaning that generating the \clock\ variable is completed.
Those agents who completed generating their \clock\ value will start propagating the maximum one they have generated. Since we use this \clock\ value for all early estimation of $\log n$, each time an agent finds out there was a greater value for the \clock\ than its own, it will reset all other computations that might have happened.

By Lemma~\ref{lem:clkvalue}, the maximum \clock\ amongst the population is a $2$ factor estimation of $\log n$. 
When any agent updates its $\clock$ with a new maximum,
it restarts the entire downstream protocol via $\reset$.
Once the maximum $\clock$ value is generated in the population,
it propagates (triggering $\reset$) by epidemic in $O(\log n)$ time.
The \clock\ variable could be used to estimate $K$, which is the number of independent additional geometric random variables each agent will generate. We also use \clock\ to set the leaderless phase clock inside each agent. At each epoch, agents will generate one new geometric random variable and propagate its maximum. All $\a$ agents counts their number of interactions in their \counter\ variable. If any agent's \counter\ reaches $\cte.\clock$, their \phase\ variable increases by one and set they $\counter =0$.

In the \sizest\ protocol, all agents in role \a\ will finally generate $K =\constantNumGrv \cdot \clock$ geometric random variable and store a sum of maximum one generated for each phase. 
For each one of the geometric random variables, agents start with $1$ and increase it as long as they interact as the sender with \f\ agents. Similar to generating the \clock\ variable, whenever, an \a\ agent interact as the receiver with an \f\ agent, generating a geometric random variable is completed and they will move on to propagate the maximum they have generated. 
Note that 
those agents who completed generating their \gr\ value will start propagating the maximum.
% only agents who completed generating a geometric random variable participate in propagating the maximum one.
Once all agents reach $\phase =\constantNumGrv \cdot \clock$ they set $\doneEST = \true$ and $\outpt = \frac{\ksum}{\phase}+1$.
% Protocols~\ref{subprotocol:timer_done},~\ref{subprotocol:epidemic_phase} are designed for simulating the timer inside each agent. 
% All $\a$ agents counts their number of interactions in their \counter\ variable.
% In the following protocol, if any agent's \counter\ reaches $\cte.\clock$, 
% it moves to the next \phase. 
We use $|\a|$, $|\f|$ for the cardinality of \a\ and \f\ agents respectively.


\begin{algorithm}[ht]
	\floatname{algorithm}{Protocol}
	\caption{$\sizest(\rec, \sen)$}
	\label{protocol:estimation}
	\begin{algorithmic}[100]		
        
		\LeftComment {initial state of agent:
		
		    $\role = \x,$
		    
    		$\counter = 0,		
    		\ksum = 0,		
    		\phase = 0,$
    		
    		$\gr = 1,
    		\clock = 1,$
		
		    $\doneC = \false, $
		    
		    $\doneG = \false, $
		    
		    $\doneEST = \false$
		}
		
    	\State{$\partition(\rec, \sen)$}
    	\If {$\rec.\role = \a $} 
    		\State{$\rec.\counter \gets \rec.\counter +1$}
		    \State{$\timerDone(\rec)$}
        \EndIf
        \If {$\sen.\role = \a $} 
    		\State{$\sen.\counter \gets \sen.\counter +1$}
    		\State{$\timerDone(\sen)$}
        \EndIf
        
        \If{\text{one agent is in state \f\ and one is in state \a}}
            \State{$\agentA \gets $ the agent in state \a}
            \If{\agentA.\doneC\ = \false}
		        \State{$\genClk(\rec, \sen)$}
		    \ElsIf{\agentA.\doneG\ = \false}
                \State{$\genGr(\rec, \sen)$}
            \EndIf
        \EndIf
        \If{\text{both agents have $\role = \a$ and $\doneG = \true$}}
            \State{$\epidemicClk(\rec, \sen)$}
		    \If{\text{both agents have $\doneG = \true$}}
		    \State{$\epidemicPhase(\rec,\sen)$}
		    \State{$\epidemicGr(\rec, \sen)$}
		    \EndIf
		    
		    \If{\sen.\doneEST}	
		        \State{$\outpt \gets \frac{\ksum}{\phase}+1
		        $}
	        \EndIf
		\EndIf
	
	\end{algorithmic}
\end{algorithm}
\begin{algorithm}[!htbp]
	\floatname{algorithm}{Subprotocol}
	\caption{$\partition(\rec, \sen)$}
	\label{subprotocol:partition}
	\begin{algorithmic}[100]
	    \LeftComment{Partition the population in two almost equal size subpopulations.}
	    
        \If {$\sen.\role = \x , \rec.\role = \x$} 
            \State{$\sen.\role \gets \a$}
		    \State{$\rec.\role \gets \f$}
		\ElsIf{$\sen.\role = \a , \rec.\role = \x$}
		    \State{$\rec.\role \gets \f$}
		\ElsIf{$\sen.\role = \f , \rec.\role = \x$}
		    \State{$\rec.\role \gets \a$}
		\EndIf
		
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
	\floatname{algorithm}{Subprotocol}
	\caption{$\genClk(\rec, \sen)$}
	\label{subprotocol:genClk}
	\begin{algorithmic}[100]
	    \LeftComment{Generate one geometric random variable for \clock.}
        \If {$\sen.\role=\a$} \Comment{This is only called if exactly one agent has \role=\a.}
            \State{$\sen.\clock \gets \sen.\clock +1$}
        \ElsIf{$\rec.\role = \a$}
            \State{$\rec.\doneC \gets \true$}
            \State{$\rec.\clock \gets \rec.\clock+2$}
		\EndIf
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
	\floatname{algorithm}{Subprotocol}
	\caption{$\epidemicClk(\agent1, \agent2)$}
	\label{subprotocol:epidemic_clk}
	\begin{algorithmic}[100]
	    \LeftComment{Maximum generated geometric variable for $\clock$ will be propagated.}
        \If {$\agent1.\clock < \agent2.\clock$} 
            \State{$\agent1.\clock \gets \agent2.\clock$}
		    \State{$\reset(\agent1)$}
		\ElsIf{$\agent2.\clock < \agent1.\clock$} 
            \State{$\agent2.\clock \gets \agent1.\clock$}
		    \State{$\reset(\agent2)$}
		\EndIf
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!htbp]
 	\floatname{algorithm}{Subprotocol}
 	\caption{$\reset(\agent)$}
 	\label{subprotocol:reset}
 	\begin{algorithmic}[100]
 	\State {$\counter \gets 0$,		
	$\ksum \gets 0$,		
	$\phase \gets 0$,		
	$\gr \gets 1$}
%  	\Comment {reset to initial state of agent}
	\State {$\doneG \gets \false$,
	$\doneEST \gets \false$}
 	  %  \State{$\agent.\counter \gets 0$ }
 	    
 	  %   \State{$\agent.\ksum \gets 0$}
 	     
 	  %    \State{$\agent.\phase \gets 0$}
 	      
 	  %    \State{$\agent.\gr \gets 1$}
		
%  		\State{$\agent.\doneG \gets \false$}
 		
%  		\State{$\agent.\doneEST \gets \false$}
 	\end{algorithmic}
 \end{algorithm}
 
\begin{algorithm}[!htbp]
	\floatname{algorithm}{Subprotocol}
	\caption{$\genGr(\rec, \sen)$}
	\label{subprotocol:genGr}
	\begin{algorithmic}[100]
	    \LeftComment{Generating one geometric random variable for \gr.}
        \If {$\sen.\role=\a$} \Comment{This is only called if exactly one agent has \role=\a.}
            \State{$\sen.\gr \gets \sen.\gr +1$}
        \ElsIf{$\rec.\role = \a$}
            \State{$\rec.\doneG \gets \true$}
		\EndIf
	\end{algorithmic}
\end{algorithm}
 
\begin{algorithm}[!htbp]
	\floatname{algorithm}{Subprotocol}
	\caption{$\epidemicGr(\agent1, \agent2)$}
	\label{subprotocol:epidemic_gr}
	\begin{algorithmic}[100]
	    \LeftComment{Maximum generated geometric variable for $\gr$ will be propagated.}
	    \If{$\agent1.\phase = \agent2.\phase$}
            \If {$\agent1.\gr < \agent2.\gr$} 
                \State{$\agent1.\gr \gets \agent2.\gr$}
    		\ElsIf{$\agent2.\gr < \agent1.\gr$} 
                \State{$\agent2.\gr \gets \agent1.\gr$}
    		\EndIf
		\EndIf
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[ht]
	\floatname{algorithm}{Subprotocol}
	\caption{$\timerDone(\agent)$}
	\label{subprotocol:timer_done}
	\begin{algorithmic}[100]
	    \LeftComment{Agents compare their \counter\ value to the specified threshold.}
        \If {$\agent.\counter = \cte\times \agent.\clock$, $\agent.\doneEST=\false$} 
            \State{$\agent.\phase \gets \agent.\phase +1$}
            \State{$\updateSum(\agent)$}
        \EndIf
		\If{$\agent.\phase = \constantNumGrv \times \agent.\clock$} 
            \State{$\agent.\doneEST \gets \true$}
		\EndIf
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
	\floatname{algorithm}{Subprotocol}
	\caption{$\epidemicPhase(\agent1, \agent2)$}
	\label{subprotocol:epidemic_phase}
	\begin{algorithmic}[100]
	    \LeftComment{The maximum \phase\ will be propagated.}
        \If {$\agent1.\phase < \agent2.\phase$} 
            \State{$\agent1.\phase \gets \agent2.\phase$}
            \State{$\updateSum(\agent1)$}
        \ElsIf {$\agent2.\phase < \agent1.\phase$} 
            \State{$\agent2.\phase \gets \agent1.\phase$}
            \State{$\updateSum(\agent2)$}
        \EndIf
	\end{algorithmic}
\end{algorithm}
 
\begin{algorithm}[!htbp]
	\floatname{algorithm}{Subprotocol}
	\caption{$\updateSum(\agent)$}
	\label{subprotocol:update_sum}
	\begin{algorithmic}[100]
            \LeftComment{The \agent\ accumulates its current value of \gr\ in \ksum\ and move to the next \phase:}
		    
		    \State{$\agent.\ksum \gets \agent.\ksum +\agent.\gr$}
		    
            \State{$\agent.\counter \gets 0$, $\agent.\gr \gets 1$}
            
            \State{$\agent.\doneG \gets \false$}
            
	\end{algorithmic}
\end{algorithm}
% \todoi{state a more general lemma that trades off probability of correctness versus state complexity. We can say something like, for all $\epsilon > 0$, the probability of error is at most $n^{-\epsilon}$, and the state complexity is $O(\log^a n)$ where $a$ is smaller if $\epsilon$ is smaller. This can be done by two machanisms:

% 1) relax the requirement that $k \geq 4 \log n$. If it is $3 \log n$, for instance, the error probability still goes to 0 as $n \to \infty$.

% MHS: In Corollary \ref{cor:sumofgeom}\ref{cor:sumofgeomConcreteK} we set $k \geq 4\log n $ to reduce our additive error.  

% 2) put a tighter upper bound on $k$ by using a more generalized Corollary~\ref{cor:half-geom-tighter-bounds} that has an error probability of $n^{-\epsilon}$ instead of $n^{-1}$.
% }
\opt{sub}{The following corollary shows that close to half of agents end up in role $\a$. A generalized Lemma and its proof appears in the appendix.
}
% \opt{final}{A proof appears in the full version.}
\opt{full}{
    The following lemma shows that close to half of agents end up in role $\a$.
    
    \begin{lemma}\label{lem:boundOnCardinalityOfA}
        Let $a > 0$.
        In the \sizest\ protocol the cardinality of agents with \a\ role is in the interval of 
        $\left[ \frac{n}{2}-a, \frac{n}{2}+a \right]$
        % $\left[ \frac{n}{2}-\sqrt{n\ln n}, \frac{n}{2}+\sqrt{n\ln n} \right]$ 
        % with probability $\geq 1-1/n^2$.
        with probability $\geq 1-e^{-2a^2/n}$.
    \end{lemma}
    \begin{proof}
        All agents in the \sizest\ protocol start in role \x. 
        In the \partition\ protocol agents will be assigned to their new roles. 
        Finally, all agents participate in the \sizest\ protocol either having role \a\ or \f. 
        Thus, after completion of the \partition\ protocol $|\a|+|\f| = n$ holds. 
        % Note that, the first rule $\x,\x \to \a,\f$ of \partition\ protocol will increase the cardinality of both \a\ and \f\, 
        % and if we restrict ourselves to this rule $|\a|=|\f|$ always holds. 
        
        The percentage of agents that change to role $\a$ is an average of the percentage 
        of $\a$'s produced by the first rule (always exactly $1/2$)
        and the percentage produced by the next two rules.
        The next two rules ensure that if the percentage of $\a$'s so far produced is greater than $1/2$,
        then $\a$ is less likely to be produced next than a fair coin flip
        (since, conditioned on the next interaction being between one $\x$ and one non-$\x$,
        the probability of producing $\a$ is exactly $\frac{|\f|}{|\a|+|\f|}$,
        i.e., smaller if there are more $\a$'s than $\f$'s),
        and vice versa.
        Thus, 
        the distribution of the percentage difference 
        $\left| \frac{|\a|}{n} - 1/2 \right|$ 
        of $\a$'s is stochastically dominated by the difference between the percentage of heads of a fair-coin binomial distribution $\mathbf{B}(n,1/2)$ and $\mathbf{B}$'s expected percentage of $1/2$.
        Therefore we can use a binomial distribution to bound the upper and lower tails of the distribution of the number of eventual $\a$'s.
        For any $a$ the Chernoff bound says for any $a > 0,$
        $\Pr{\mathbf{B}(n, 1/2) \geq n/2 + a} \leq e^{-2a^2/n}$
        and 
        $\Pr{\mathbf{B}(n, 1/2) \leq n/2 - a} \leq e^{-2a^2/n}$.
    \end{proof}
}

\begin{corollary}\label{cor:lazyboundOnCardinalityOfA}
    In the \sizest\ protocol the cardinality of agents with \a\ role is in the interval of 
    $\left[ \frac{n}{3}, \frac{2n}{3} \right]$
    with probability $\geq 1-e^{-n/18}$.
\end{corollary}

The following corollary shows that generating one geometric random variable takes $O(\ln n)$ with high probability.
\opt{sub}{A generalized Lemma with a proof appears in the appendix.}
\opt{full}{
\begin{lemma}\label{lem:timeToGenerateGR}
    Let $\alpha>0$.
    With probability $\geq 1 - (3/n)^{\alpha-1} - 2 e^{-n/18}$,
    each of protocols \genClk\ and \genGr\ require at most $4\alpha \ln n$ time 
    for all agents to generate one geometric random variable.
\end{lemma}
\begin{proof}
    In this proof, we use the facts,
    following from Corollary~\ref{cor:lazyboundOnCardinalityOfA},
    that $|\a| \geq n/3$ with probability $\geq 1 - e^{-n/18}$,
    and similarly for $|\f| \geq n/3$.
    We model time for generating all geometric random variables as the time to collect all $|\a|$ coupons in a modified coupon problem.
    In the modified problem,
    after $i-1$ coupons have been collected,
    the probability of collecting the $i$'th coupon on the next try,
    rather than being $p_i = \frac{1}{i-1}$,
    is instead 
    $p_i 
    = \frac{|\a-(i-1)| \cdot |\f| \cdot 1/2}{\binom{n}{2}}
    = \frac{|\a-(i-1)| \cdot |\f|}{n(n-1)}$.
    This models that the two agents must be in roles $\a$,$\f$, respectively,
    and the agent in role $\a$ must be the receiver, 
    to complete the generating of the $\a$ agent's geometric random variable.
    Let $\mathbf{T}$ be the time to collect all $|\a|$ coupons, and let $\mathbf{t}_i$ be the time to collect the $i$'th coupon after $i-1$ coupons have been collected,
    with $\E{\mathbf{t}_i} = 1 / p_i$. 
    Then
    \begin{eqnarray*}
            \E{\mathbf{T}}
        &=&
            \sum_{i=1}^{|\a|} \E{\mathbf{t}_i} 
        =
            \sum_{i=1}^{|\a|} \frac{1}{p_i}
        =%\\&=&
            \sum_{i=1}^{|\a|} \frac{n(n-1)}{|\f|\cdot|\a-(i-1)|}
        \\&=&           \frac{n(n-1)}{|\f|}\sum_{i=1}^{|\a|} \frac{1}{i}
        \leq %\\&\leq&
            \frac{n(n-1) H_{|\a|}}{|\f|}
        \\&\leq&
            \frac{n(n-1) H_{|\a|}}{\frac{n}{3}} 
            \ \ \ \ \ \text{since $|\f| \geq \frac{n}{3}$ by Corollary~\ref{cor:lazyboundOnCardinalityOfA}}
        \\&=&
            3 (n-1) H_{|\a|}.
    \end{eqnarray*}
    For the upper bound, 
    fix some coupon that has not been collected 
    ($\a$ agent that has not completed its geometric random variable).
    The probability that the next interaction collects \emph{that} coupon is $\frac{|\f|}{2 \binom{n}{2}}$.
    If $T_m = 3 \alpha (n-1)\ln{|\a|}$,
    then the probability of that not getting selected after $T_m$ time is then
    $= \left(1- \frac{|\f|}{2\cdot \binom{n}{2}}\right)^{T_m}\leq \left(1- \frac{n}{3n(n-1)}\right)^{T_m}$. 
    By the union bound over all agents in role \a, the probability that there exists a coupon that is not selected after $T_m$ time is 
    $\leq |\a| \left(1- \frac{1/3}{n-1} \right)^{\alpha \cdot 3(n-1)\ln{|\a|}} 
    \leq |\a| e^{- \alpha \ln {|\a|} } 
    = \frac{1}{|\a|^{\alpha-1}} 
    \leq \left( \frac{3}{n} \right)^{\alpha-1}$,
    where the last inequality follows from $|\a| \geq n/3$ with probability $\geq 1 - e^{-n/18}$.
\end{proof}
}
Setting $\alpha =3$ in Lemma~\ref{lem:timeToGenerateGR} gives the following.

\begin{corollary}\label{cor:exacttimeToGenerateGR}
Protocols \genClk\ and \genGr\ require at most $12 \ln n$ time to generate one geometric random variable with probability $\geq 1 - \frac{9}{n^{2}}- 2e^{-n/18}$.
\end{corollary}

In each epoch, one geometric random variable 
(in the first epoch \clock\ and in the subsequent epochs \gr) 
is generated and its maximum will be propagated by epidemic among the population. We set the time of each epoch equal to the required time of generating one plus the time for completion of an epidemic.
To analyze the time complexity of our protocol, 
we require the time bounds for completing an epidemic from the paper~\cite{AAE08}. 
The current form is taken from~\cite{doty2018exact}.
For all $n \in \N^+$,
let $H_n = \sum_{k=1}^n \frac{1}{k}$ denote the $n$'th harmonic number.
Note that $\ln n \leq \frac{n-1}{n} H_{n-1} \leq 1 + \ln n$.

% \begin{lemma}[\cite{AAE08}]\label{lem:epidemic}
% Suppose an epidemic happens among a population of $n$ agents.
% Let $T$ denote the time to complete such an epidemic.
% Then
% $\E{T} \leq \epidemicExpectedTimeConstant \ln n$,
% $\Pr{T < \frac{1}{4} \ln n} < 2 e^{-\sqrt{n}}$,
% and for any $\alpha_u > 0$,
% $\Pr{T > \alpha_u \ln n} < n^{- \alpha_u/4+1}$.
% \end{lemma}
\opt{final}{
\begin{lemma}[\cite{AAE08}]\label{lem:epidemic}
Let $T$ denote the time to complete an epidemic.
Then
$\E{T} = \frac{n-1}{n} H_{n-1}$,
$\Pr{T < \frac{1}{4} \ln n} < 2 e^{-\sqrt{n}}$,
and for any $\alpha_u > 0$,
$\Pr{T > \alpha_u \ln n} < 4 n^{- \alpha_u/4+1}$.
\end{lemma}
}

The following corollary describes an epidemic in a subpopulation.
This refers to some subset $S$ of the population executing epidemic transitions only among themselves,
which slows down the epidemic by only a constant factor if $|S| = \Omega(n)$.

\opt{full}{
\begin{corollary}\label{cor:partialEpidemic}
    Let $c \geq 1$.
    Suppose an epidemic happens among a subpopulation of $a = n/c$ agents.
    Let $\mathbf{T}$ denote the time to complete such an epidemic.
    Then
    for any $\alpha_u > 0$,
    $\Pr{\mathbf{T} > \alpha_u \ln a} < a^{ -(\alpha_u-4c)^2 / 12c }$.
\end{corollary}
\begin{proof}
    The probability that in the next interaction the scheduler picks two agents from the subpopulation $a$ is $\binom{a}{2} / \binom{n}{2} = \frac{a(a-1)}{n(n-1)}$. 
    By Lemma~\ref{lem:epidemic}, 
    if $\mathbf{T}'$ denotes the time to complete an epidemic in population size $a$, 
    then $\E{\mathbf{\mathbf{T}}'} = \frac{a-1}{a} H_{a-1}$. 
    Since we have $\frac{n(n-1)}{a(a-1)}$ expected interactions in the whole population of size $n$
    in order to obtain one interaction within the subpopulation,
    the expected time to complete this epidemic (counting total interactions in the whole population)
    is $\E{\mathbf{T}} = \frac{n(n-1)}{a(a-1)} \cdot \E{\mathbf{T}'} = \frac{n(n-1)}{a(a-1)} \frac{a-1}{a}H_{a-1} = \frac{n(n-1)}{a^2}H_{a-1} \geq c^2 \ln a.$ 
    % $\frac{\binom{a}{2}}{\binom{n}{2}}=\frac{n-c}{c^2(n-1)}$. 
    % By Lemma~\ref{lem:epidemic}, 
    % if $\mathbf{T}'$ denotes the time to complete an epidemic in population size $a$, 
    % then $\E{\mathbf{\mathbf{T}}'} = \frac{a-1}{a} H_{a-1}$. 
    % Since we have $c^2(n-c)/(n-1)$ expected interactions in the whole population of size $n$
    % in order to obtain one interaction within the subpopulation,
    % the expected time to complete this epidemic (counting total interactions in the whole population)
    % is $\E{\mathbf{T}} = c^2 \frac{n-1}{n-c} \cdot \E{\mathbf{T}'} = c^2 \frac{(n-1)(a-1)}{a(n-c)}H_{a-1} \geq c^2H_{a-1}$. 
    By the Chernoff bound we have:
    \begin{eqnarray*}
        \Pr{\mathbf{T} \geq (1+\delta)\E{\mathbf{T}}}
    &\leq&
        e^{-\delta^2 \E{\mathbf{T}} / 3}
    \\&\leq&
        e^{-\delta^2 \cdot c^2 \ln(a) / 3}
    \\&=&
        a^{-c^2\delta^2 / 3} 
    \end{eqnarray*}
    Setting $\alpha_u = 4c(1+\delta)$, 
    $\Pr{\mathbf{T} \geq \alpha_u \ln a} \leq
    a^{ -((\alpha_u/4c)-1)^2c^2 / 3 }$.
    % We can conclude with probability $\geq 1-\frac{1}{n^3}$ an epidemic takes 
    % $\leq 54 \ln n$ time to complete within the subpopulation of size $a$.
\end{proof}
}
Setting $c=3$ and $\alpha_u = 24$ in Corollary~\ref{cor:partialEpidemic} gives the following.
\begin{corollary}\label{cor:partialEpidemic-c-equals-3}
    Suppose an epidemic happens among a subpopulation of $n/3$ agents with time $\mathbf{T}$.
    Then $\Pr{\mathbf{T} > 24 \ln n} < 27 n^{-3}$.
\end{corollary}

By Corollaries~\ref{cor:exacttimeToGenerateGR}, Corollary~\ref{cor:partialEpidemic-c-equals-3} we can obtain the following corollary.

\begin{corollary}\label{cor:generateGRplusEpidemic}
    Suppose at lease $n/3$ agents are in role \a.
    Let $\mathbf{T}$ be the time for them generate one geometric random variable 
    and propagate its maximum to the whole subpopulation of $\a$'s.
    Then $\Pr{\mathbf{T} > 36 \ln n} < 10n^{-2}$.
\end{corollary}

The next lemma bounds the number of interactions an agent has in a given time,
and it is the basis of the leaderless phase clock we use.
\opt{sub}{It is proven in the appendix.}
\opt{final}{It is proven in~\cite{doty2018efficientArxiv}.}
It follows from a simple Chernoff bound on the number of interactions involving a single agent in a given window of time.


\restateableLemma{lem:boundONepoch}{LemBoundOnepoch}{
    Let $C \geq 3$ and $D = 2C + \sqrt{12 C}$.
    In time $C \ln n $, with probability $\geq 1-1/n$, 
    each agent has at most $D \ln n$ interactions.
}{
    Fix an agent $a$.
    Let $\mathbf{I}_a$ be the number of interactions involving $a$ during  $C n\ln n$ total interactions ($C \ln n$ time).
    The probability that any given interaction involves $a$ (either receiver or sender) is exactly $\frac{2}{n}$, 
    so $\mathbf{I}_a$ is distributed binomially, and
    $\E{\mathbf{I}_a} = C n \ln n \cdot \frac{2}{n} = 2 C \ln n$. 
    Applying the Chernoff bound,
    for any $0 < \delta \leq 1$,
    \[
        \Pr{\mathbf{I}_a \geq (1+\delta) 2C\ln n} 
    \leq
        e^{-\delta^2 2C\ln(n) / 3}
    =
        n^{-2C\delta^2 / 3}.
    \]
    Let $D = 2C + \sqrt{12 C}$,
    and let $\delta = \frac{D}{2C} - 1$.
    (Note $\delta \leq 1$ so long as $C \geq 3$.)
    Then $(1+ \delta) 2C \ln n = D \ln n$
    and
    $n^{-2C\delta^2 / 3} = n^{\frac{-(D-2C)^2}{6C}} = n^{-2}$.
    Then 
    $
        \Pr{\mathbf{I}_a \geq D \ln n} \leq
    n^{-2}.
    $
    By the union bound,
    $
        \Pr{(\exists a)\ \mathbf{I}_a \geq D\ln n} 
    \leq
        n^{-1}.
    $
    So, by setting $D = 2C+ \sqrt{12C}$ we bound the probability that each agent has more than $D \ln n$ interactions in time $C \ln n $ to be $\leq 1/n$.
}

\opt{full}{\proofLemBoundOnepoch}

\begin{corollary}\label{cor:exactboundonepoch}
Each agent has $\geq 96 \ln n$ interactions
in time $36 \ln n$
with probability $\leq 1/n$.
\end{corollary}

By Lemma~\ref{lem:boundONepoch} each agent has at most 
$\left(2\cdot 36 +\sqrt{12 \cdot 36}\right) \ln n \leq 96 \ln n \leq 139 \log n$ interactions in the time that it takes to generate and propagate maximum of one geometric random variable. 
Thus, each agent should count up to $139 \log n$ for its leaderless phase clock,
to ensure that with high probability none reaches that count until the maximum geometric random variable is known to all agents. 
However, agents are not aware of any approximation of $\log n$. In the \sizest\ protocol, agents use their \clock\ variable for this approximation. 
As mentioned, all the agents in role \a\ start by generating one geometric random variable \clock.
The maximum in the population is used as a weak (constant factor) approximation of $\log n$. 
\opt{full}{
Corollary~\ref{cor:half-geom-tighter-bounds} says that the maximum of $|\a|$ geometric random variables is in the interval of
$[\log |\a| - \log \ln |\a|, 2\log |\a|]$ 
with probability at least $1-1/|\a|$. However, we are using the \clock\ and \gr\ variables as an approximation of $\log n$ rather than $\log |\a|$. Lemma~\ref{lem:clkvalue} will give us a bound over the \clock\ value with respect to $\log n$. Corollaries~\ref{cor:grvalue},~\ref{cor:boundONtime},~\ref{cor:boundONcoefficient} use this lemma for a bound over \gr, \counter, and \phase\ values.
}
\opt{sub}{Their statement and proofs appear in the appendix.}
\opt{final}{Their statement and proofs appear in~\cite{doty2018efficientArxiv}.}
\opt{full}{
\begin{lemma}\label{lem:clkvalue}
    The \clock\ value generated by \genClk\ is in the interval of $[\log n - \log \ln n, 2\log n+1]$ with probability at least $1-1/n-e^{-n/18}$.
\end{lemma}
\begin{proof}
    
    By Corollary~\ref{cor:lazyboundOnCardinalityOfA}, $n/3\leq |\a| \leq 2n/3$ with probability $\geq 1-e^{-n/18}$. We apply the result of Corollary~\ref{cor:half-geom-tighter-bounds} and substitute $n$ with $|\a|$:
    \begin{alignat*}{2}
    \log {(n/3)} - \log \ln {(n/3)}
    &\leq 
    \clock 
    &\leq 
    2\log {(2n/3)}\\
    \log n -1.6 - \log \ln n -0.4
    &\leq 
    \clock 
    &\leq 
    2\log n + 2\log (2/3)\\
    \log n - \log \ln n -2
    &\leq 
    \clock 
    &\leq 
    2\log n-1\\
    \log n - \log \ln n -2
    &\leq 
    \clock 
    &\leq 
    2\log n-1
    \end{alignat*}
    So, by setting $\clock = \clock +2$ for all agents, this variable is in the interval of $[\log n -\log \ln n , 2\log n + 1]$ with probability $\geq 1-1/n-e^{-n/18}$.
\end{proof}
}

%\opt{full}{\proofLemClkValue}

\opt{final}{
    \begin{corollary}\label{cor:grvalue}
    The \gr\ value generated by \genGr\ is in the interval of $[\log n - \log \ln n-2, 2\log n-1]$ with probability at least $1-1/n-e^{-n/18}$.
    \end{corollary}
    
    \begin{corollary}\label{cor:boundONtime}
    The number of interactions in each epoch in the $\sizest$ is in the interval 
    $[\cte \log n - \cte \log \ln n, 281\log n]$ with probability $\geq 1-1/n-e^{-n/18}$. \end{corollary}
    
    \begin{proof}
    By Corollary~\ref{cor:exactboundonepoch}, agents should count up to $96\ln \leq 139 \log n$ before moving to the next epoch. if we set the threshold of the \counter\ to $\cte \cdot \clock$, $\cte \log n - \cte  \log \ln n \geq 139 \log n$ then the \counter\ variable will be in the interval of $[\cte \log n - \cte \log \ln n, 280\log n+\cte]$ with high probability ($280 \log n + \cte \leq 281 \log n$ for $n \geq 2$).
    \end{proof}
    
    \begin{corollary}\label{cor:boundONcoefficient}
    The number of epochs in the $\sizest$ is in the interval 
    $[\constantNumGrv\log n - \constantNumGrv\log \ln n, 11\log n]$ with probability $\geq 1-1/n-e^{-n/18}$. \end{corollary}
    
    \begin{proof}
    By Corollary~\ref{cor:sumofgeomConcreteK}, to achieve the additive error of \logSizeError\ for our protocol the number of geometric random variables should be $\geq 4\log n$. By setting the threshold of the number of phases to $\constantNumGrv \times \clock$, for $n\geq 200$, $\constantNumGrv \log n - \constantNumGrv \log \ln n \geq 4\log n$. The number of phases will be in the interval of $[\constantNumGrv\log n - \constantNumGrv\log \ln n, 10\log n + \constantNumGrv]$ with high probability ($10 \log n + \constantNumGrv\leq 11 \log n$ for $n\geq 2$).
    \end{proof}
}







The next Lemma bounds the space complexity of our main protocol
by counting the likely range taken by the variables in $\sizest$.
\opt{sub,final}{
    It is proven 
    \opt{sub}{in the Appendix.}
    \opt{final}{in~\cite{doty2018efficientArxiv}.}
}

\restateableLemma{lem:space}{LemSpace}{
    $\sizest$ uses $O(\log^\numStatesExponent n)$ states with probability $\geq 1-O(\log n)/n$.
}{
    With probability at least $1 - O(1/n)$
    (see individual lemma statements for constants in the $O$),
    the set of values possibly taken on by each field are given as follows:
    \begin{center}
    \begin{tabular}{ l l l }
     \clock & $\{1, \ldots, 2\log n+1\}$ 
            & Lemma~\ref{lem:clkvalue} \\ 
     \gr & $\{1, \ldots, 2\log n\}$ 
            & Corollary~\ref{cor:grvalue} \\ 
     \phase & $\{0,\ldots, 11 \log n\}$ 
            & Corollary~\ref{cor:boundONcoefficient} \\
     \counter & $\{0, \ldots, 281 \log n\}$ 
            & Corollary~\ref{cor:boundONtime} \\
     \ksum & $\{0, \ldots, 22 \log ^2 n\}$ 
            & Corollaries~\ref{cor:grvalue},~\ref{cor:boundONcoefficient}
    \end{tabular}
    \end{center}
    
    After each agent sets $\doneEST =\true$, 
    it no longer needs to store the value in \gr\ and can use that space to store the result of $\ksum / \phase +1$ as the output. The probability that each geometric random variable is greater than $2\log n$ is less than $1/n$, by the union bound the probability that any of them is greater than $2\log n$ is less than $\frac{11\log n}{n}$.
}

\opt{full}{\proofLemSpace}




The next corollary bounds the time complexity of protocol \sizest;
the main component of the time complexity is that $\Theta(\log n)$ geometric random variables must be generated and propagated by epidemic among the population,
each epidemic taking $\Theta(\log n)$ time.
\opt{sub}{A proof appears in the appendix.}
\opt{final}{A proof appears in~\cite{doty2018efficientArxiv}.}
\restateableCorollary{cor:timecomplexity}{CorTimeComplexity}{
    The \sizest\ protocol take $O(\log^2 n)$ time with probability at least $1-1/n$ for all agents set $\doneEST =\true$.
}{
    By Corollary~\ref{cor:generateGRplusEpidemic}, with probability $\geq 1-(10/n^2)$ generating and propagating the maximum of the \clock\ variable takes at most $36\ln n$ time.
    
    By Corollary~\ref{cor:boundONcoefficient}, at most $11 \log n$ geometric random variables will be generated, 
    and by Corollary~\ref{cor:generateGRplusEpidemic}, with probability $\geq 1-(10/n^2)$ a given variable takes at most $36\ln n$ time to generate and propagate its maximum (total of $11 \log n\cdot36 \ln n$ time).
    
    By the union bound over all epochs, 
    the probability that generating $11 \log n +1 $ geometric random variables and propagating their maximum takes more than $(11\log n +1) \cdot 36 \ln n$ time is $\geq 1- \frac{O(\log n)}{n^2} \geq 1-1/n$ for large values of $n$.
}
\opt{full}{\proofCorTimeComplexity}
\opt{sub}{Finally, the following corollary bounds the \outpt\ produced by \sizest\ protocol. A proof appears in the appendix.}
\restateableCorollary{cor:sumofgeometricamongAagents}{CorSumOfGeometricAmongAagents}{
    Let $K \geq 4\log n$ and $a$ be the number of agents in role \a. 
    Let $\ksum/K$ be the average of $K$ geometric random variables in \sizest. Then $\Pr{ \left| \frac{\ksum}{K}+1 - \log n \right| \geq \logSizeErrorAagents } 
        \leq \frac{6}{n}$.
}{
        By Corollary~\ref{cor:sumofgeomConcreteK}, 
    $
            \Pr{ \left| \frac{\ksum}{K} - \log a \right| \geq \logSizeError } 
        \leq 
            \frac{2}{a}.
     $ By Lemma~\ref{lem:boundOnCardinalityOfA}, $  \frac{n}{2}-\sqrt{n\ln n} \leq a \leq \frac{n}{2}+\sqrt{n\ln n}$. So, $\log n -2 \leq \log a \leq \log n$. Hence, by setting $\frac{\ksum}{K}+1$ as the output of \sizest\ protocol:
     $
            \Pr{ \left| \frac{\ksum}{K}+1 - \log n \right| \geq \logSizeError+1 } 
        \leq 
            \frac{2}{a} \leq \frac{6}{n}.
     $
    }
\opt{full}{
\proofCorSumOfGeometricAmongAagents
}
\opt{full}{
Finally, 
we combine these results to prove the main result of this section.
\proofTHMmainSizeEstimationProtocol
}

%\todoi{justify that $K = 4 \sqrt{\log n}$ parallel epidemics finish quickly. Do this with a general lemma for any $K$ and have a $K = 4 \sqrt{\log n}$ corollary. I commented out a start of an attempt below, but stopped when I remembered that the epidemics are not independent. We can get an easy bound of $K \log n$ by bounding the maximum by the sum, and maybe we can get fancy later and try some tricks that work on dependent random variables, although most of those techniques require the variables to be bounded, so I don't want to spend too much time thinking about it. A running time of $4 \sqrt{\log n} \log n = 4 \log^{1.5} n$ is still very good. It may be worth seeing if we have negative dependence: if the dependence between epidemics causes them to finish faster than they would if they were independent. If so we can apply Chernoff.}

%\todoi{add corollary that leader election and majority have uniform protocols, with the proof explaining how to compose them (describe restarting condition of putting an agent running the leader election subprotocol back into that subprotocol's initial state whenever the average $X/K$ changes.)}








% We require the following lemma,
% first proven by Angluin, Aspnes, TODO~\cite{AAE06}.
% The current form is taken from~\cite{exact-size-counting}.

% \begin{lemma}[\cite{AAE08}]\label{lem:epidemic}
%     Let $T$ denote the time to complete an epidemic.
%     Then
%     $\E{T} \leq \epidemicExpectedTimeConstant \ln n$,
%     $\Pr{T < \frac{1}{4} \ln n} < 2 e^{-\sqrt{n}}$,
%     and for any $\alpha_u > 0$,
%     $\Pr{T > \alpha_u \ln n} < 4 n^{- \alpha_u/4+1}$.
% \end{lemma}

% \begin{corollary}
%     Let $T$ denote the time to complete an epidemic.
%     Let $\alpha_L = ??, \beta_L = ??, \alpha_U = ??, \beta_U = ??$.
%     Then for all $t > 0$
%     $\Pr{T < t} < \alpha_L e^{- \beta_L t}$,
%     and 
%     $\Pr{T > t} < \alpha_U n^{- \beta_U t}$.
% \end{corollary}

% \begin{proof}
%     \todoi{TODO}
% \end{proof}

% \todo{
% With this,
% we can prove that $K$ independent epidemics complete quickly by bounding the time for each by an exponential,
% and then just analyzing the maximum of the exponentials.
% }



